Performance-Driven Cascade Controller Tuning with Bayesian Optimization

We propose a performance-based autotuning method for cascade control systems, where the parameters of a linear axis drive motion controller from two control loops are tuned jointly. Using Bayesian optimization as all parameters are tuned simultaneously, the method is guaranteed to converge asymptotically to the global optimum of the cost. The data-efficiency and performance of the method are studied numerically for several training configurations and compared numerically to those achieved with classical tuning methods and to the exhaustive evaluation of the cost. On the real system, the tracking performance and robustness against disturbances are compared experimentally to nominal tuning. The numerical study and the experimental data both demonstrate that the proposed automated tuning method is efficient in terms of required tuning iterations, robust to disturbances, and results in improved tracking.

==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/author_block.tex <==
%\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
%\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\textit{name of organization (of Aff.)}\\
%City, Country \\
%email address}
%\and
%\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
%\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\textit{name of organization (of Aff.)}\\
%City, Country \\
%email address}
%\and
%\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
%\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
%\textit{name of organization (of Aff.)}\\
%City, Country \\
%email address}

\author{\IEEEauthorblockN{
Mohammad Khosravi, Varsha Behrunani, Piotr Myszkorowski, Roy S. Smith, Alisa Rupenyan and John Lygeros}% <-this % stops a space
\thanks{The authors are with the Automatic Control Laboratory, ETH Z\"urich. A. Rupenyan is also with inspire AG, 8092 Z\"urich, Switzerland. (e-mails: \{khosravm, bvarsha,	rsmith, ralisa, lygeros\}@control.ee.ethz.ch). P. Myszkorowski is with Sigmatek AG, piotr.myszkorowski@sigmatek.ch.
} 
}


==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/mystyle.tex <==
%===================== Packages ====================
%\usepackage[numbers]{natbib}
%\usepackage{natbib}
%\usepackage[noadjust]{cite}
%\usepackage[colorlinks=true]{hyperref}
\usepackage{amssymb, amsmath, amsfonts}
\usepackage{  mathrsfs, color, bm,bbm}%, url,authblk,dsfont,
\usepackage{ graphicx, epstopdf}%, subfigure}%, subcaption}% , transparent,, pgfplots
\usepackage{algorithm,  multirow,titlecaps,algorithmicx}
\usepackage[T1]{fontenc}

%\usepackage{threeparttable}

\usepackage{tikzsymbols}
% Defining mathbbold font
\DeclareMathAlphabet{\mathbbold}{U}{bbold}{m}{n}

% For pseudocodes and algorithms
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[noend]{algpseudocode} 
%=================================================
%\usepackage{cite}
\usepackage{amsmath,amssymb,amsfonts}
%\usepackage{algorithmic}
\usepackage{graphicx}
%\usepackage{textcomp}
\usepackage{xcolor}
%\usepackage{hyperref}
% for nice tables ...
%\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{courier}
\usepackage{float}
\usepackage{makecell}
\setcellgapes{5pt}
%\usepackage{subcaption}
%\captionsetup{compatibility=false}
%\usepackage[options ]{algorithm2e}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
%\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
%		T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}
%==================== Commenting ==================
\newcommand{\cm}[1]{{\color{violet}{{[#1]}}}}
\newcommand{\cmb}[1]{{\color{blue}{#1}}}
\newcommand{\cmr}[1]{{\color{red}{#1}}}
\newcommand{\cmg}[1]{{\color{green}{#1}}}
\newcommand{\cmm}[1]{{\color{magenta}{#1}}}
\newcommand{\cmc}[1]{{\color{cyan}{#1}}}
\newcommand{\cmt}[1]{{\color{teal}{#1}}}
\newcommand{\cmp}[1]{{\color{purple}{#1}}}
%=================================================
\newcommand{\stiny}[1]{{\scalebox{.5}{#1}}}
\newcommand{\smtiny}[1]{{\scalebox{.63}{#1}}}
\newcommand{\sstiny}[1]{{\scalebox{.25}{#1}}}
%================= MATH Abbreviation ==============
%=============== Abbreviation ==================
\newcommand{\argmin}{{\mathrm{argmin}}}
\newcommand{\argmax}{{\mathrm{argmax}}}
\newcommand*{\argminOp}{\operatornamewithlimits{argmin}\limits}
\newcommand*{\argmaxOp}{\operatornamewithlimits{argmax}\limits}
\newcommand*{\minOp}{\operatornamewithlimits{min}\limits}
\newcommand*{\maxOp}{\operatornamewithlimits{max}\limits}
\newcommand*{\sumOp}{\operatornamewithlimits{\sum}\limits}
\newcommand*{\supOp}{\operatornamewithlimits{sup}\limits}
\newcommand*{\infOp}{\operatornamewithlimits{inf}\limits}
\newcommand{\Max}{\max\limits}
\newcommand{\Min}{\min\limits}
\newcommand{\Sup}{\sup\limits}
\newcommand{\Inf}{\inf\limits}
\newcommand{\Sum}{\sum\limits}
\newcommand{\GP}[2]{{\mathcal{G}\!\mathcal{P}}(#1,#2)}
\newcommand{\ddt}[1]{\frac{\mathrm{d}}{\mathrm{d}t}#1}
\newcommand{\tr}{{\mathsf{T}}}
\newcommand{\Hr}{{\mathsf{H}}}
\newcommand{\zero}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\iftrue%\iffalse %<-<-<-<-<-<-<-<-<-<-<-<-<-<-<
\newcommand{\zeromx}{{\mathbbold{0}}} %<<<<
\newcommand{\eye}{\mathbb{I}}
\else
\newcommand{\zeromx}{{\mathbf{0}}} %<<<<
\newcommand{\eye}{\mathbf{I}}
\fi%<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<-<
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\vc}[1]{{ \mathrm{#1} }}
\newcommand{\vcc}[1]{{ \mathrm{\mathbf{#1}} }}
\newcommand{\mx}[1]{{ \mathrm{#1} }}
\newcommand{\mxx}[1]{{ \mathrm{\mathbf{#1}} }}
\newcommand*{\Times}{\operatornamewithlimits{\scalebox{1.5}{$\times$}}\limits} % large x or times
\newcommand{\dom}{\mathrm{dom}}	% domain of a function
\newcommand{\conv}{\mathrm{conv}} % convex hull
\newcommand{\convcone}{\mathrm{convcone}} % convex hull
\newcommand{\pos}{\mathrm{pos}} % positive hull
\newcommand{\supp}{\mathrm{supp}} % positive 
\newcommand{\diag}{\mathrm{diag}}
\newcommand{\Diag}{\mathrm{Diag}}
\newcommand{\closure}{\mathrm{cl}} %closure
\newcommand{\interior}{\mathrm{int}} %closure
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\inner}[2]{{ \langle {#1,#2} \rangle}}
\newcommand{\imag}[1]{\mathrm{imag}(#1)}
\newcommand{\nth}{{\text{\tiny{th}}}}
\newcommand{\trace}{\mathrm{tr}}

%% __ mathscr of D, F, X, Y, Z,...
\newcommand{\Ascr}{{\mathscr{A}}}
\newcommand{\Bscr}{{\mathscr{B}}}
\newcommand{\Cscr}{{\mathscr{C}}}
\newcommand{\Dscr}{{\mathscr{D}}}
\newcommand{\Escr}{{\mathscr{E}}}
\newcommand{\Fscr}{{\mathscr{F}}}
\newcommand{\Gscr}{{\mathscr{G}}}
\newcommand{\Hscr}{{\mathscr{H}}}
\newcommand{\Iscr}{{\mathscr{I}}}
\newcommand{\Jscr}{{\mathscr{J}}}
\newcommand{\Kscr}{{\mathscr{K}}}
\newcommand{\Lscr}{{\mathscr{L}}}
\newcommand{\Xscr}{{\mathscr{X}}}
\newcommand{\Yscr}{{\mathscr{Y}}}
\newcommand{\Zscr}{{\mathscr{Z}}}

%% __ mathcal of X, Y, Z,...
\newcommand{\Acal}{{\mathcal{A}}}
\newcommand{\Bcal}{{\mathcal{B}}}
\newcommand{\Ccal}{{\mathcal{C}}}
\newcommand{\Dcal}{{\mathcal{D}}}
\newcommand{\Ecal}{{\mathcal{E}}}
\newcommand{\Fcal}{{\mathcal{F}}}
\newcommand{\Gcal}{{\mathcal{G}}}
\newcommand{\Hcal}{{\mathcal{H}}}
\newcommand{\Ical}{{\mathcal{I}}}
\newcommand{\Jcal}{{\mathcal{J}}}
\newcommand{\Kcal}{{\mathcal{K}}}
\newcommand{\Lcal}{{\mathcal{L}}}
\newcommand{\Mcal}{{\mathcal{M}}}
\newcommand{\Ncal}{{\mathcal{N}}}
\newcommand{\Ocal}{{\mathcal{O}}}
\newcommand{\Pcal}{{\mathcal{P}}}
\newcommand{\Qcal}{{\mathcal{Q}}}
\newcommand{\Rcal}{{\mathcal{R}}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{{\mathcal{U}}}
\newcommand{\Wcal}{{\mathcal{W}}}
\newcommand{\Xcal}{{\mathcal{X}}}
\newcommand{\Ycal}{{\mathcal{Y}}}
\newcommand{\Zcal}{{\mathcal{Z}}}

%% __ mathbb of X, Y, Z,...
%\newcommand{\Bbb}{{\mathbb{B}}}
\newcommand{\Cbb}{{\mathbb{C}}}
\newcommand{\Dbb}{{\mathbb{D}}}
\newcommand{\Ebb}{{\mathbb{E}}}
\newcommand{\Fbb}{{\mathbb{F}}}
\newcommand{\Gbb}{{\mathbb{G}}}
\newcommand{\Hbb}{{\mathbb{H}}}
\newcommand{\Ibb}{{\mathbb{I}}}
\newcommand{\Jbb}{{\mathbb{J}}}
\newcommand{\Kbb}{{\mathbb{K}}}
\newcommand{\Lbb}{{\mathbb{L}}}
\newcommand{\Mbb}{{\mathbb{M}}}
\newcommand{\Nbb}{{\mathbb{N}}}
\newcommand{\Pbb}{{\mathbb{P}}}
\newcommand{\Qbb}{{\mathbb{Q}}}
\newcommand{\Rbb}{{\mathbb{R}}}
\newcommand{\Sbb}{{\mathbb{S}}}
\newcommand{\Tbb}{{\mathbb{T}}}
\newcommand{\Ubb}{{\mathbb{U}}}
\newcommand{\Vbb}{{\mathbb{V}}}
\newcommand{\Xbb}{{\mathbb{X}}}
\newcommand{\Ybb}{{\mathbb{Y}}}
\newcommand{\Zbb}{{\mathbb{Z}}}
\newcommand{\bbo}{\mathbbold{o}}
%\newcommand{\bbo}{\mathbb{o}}
\newcommand{\bbh}{\mathds{h}}
%\newcommand{\bbk}{\mathds{k}}
%\newcommand{\bbk}{\mathbbold{k}}
\newcommand{\bbk}{\mathbbm{k}}

%% __ hat of f, g
\newcommand{\hatf}{{\hat{f}}}
\newcommand{\hatg}{{\hat{g}}}
%_______________________________________________
\newcommand{\SumN}{\sum\limits_{i=1}^N}
\newcommand{\WWbar}{\widetilde{\mathbb{W}}}

%% __ other fonts (Probability)
\newcommand{\PP}{\mathds{P}}
\newcommand{\QQ}{\mathds{Q}}
\newcommand{\EE}{\mathds{E}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\WW}{\mathbb{W}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\XX}{\mathbb{X}}
\newcommand{\FF}{\mathcal{F}}
\newcommand{\KK}{\bm{\mathcal{K}}}
\newcommand{\GG}{\bm{\mathcal{G}}}
\newcommand{\II}{\mathcal{I}}
\newcommand{\JJ}{\mathcal{J}}
\newcommand{\LL}{\mathcal{L}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\NN}{\mathcal{N}}
\newcommand{\ZZ}{\mathcal{Z}}

%==================================================
%===================== Theorem ====================
\newtheorem{theorem}{Theorem}[section]
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{proposition}[theorem]{Propositon}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
%==================================================
%==================== Figures Path ================
%\graphicspath{{figures/}}
%==================================================
%===================== TODO List ==================
%\iftrue %<--
\iffalse
\let\labelindent\relax
\usepackage{enumitem}
\newlist{todolist}{itemize}{2}
\setlist[todolist]{label=$\square$}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%
\newcommand{\done}{\rlap{$\square$}{\raisebox{2pt}{\large\hspace{1pt}\cmark}}% 
	\hspace{-2.5pt}}
% for being done and remain in list!
\newcommand{\wontfix}{\rlap{$\square$}{\large\hspace{1pt}\xmark}} 
% for being conceled but remain in the list!
\fi 
%=================================================
%==== Modify style ===============================
%\iftrue %<--
\iffalse
	\usepackage{xcolor}
	\hypersetup{
		colorlinks,
		linkcolor={blue!55!black},
		citecolor={red!55!black},
		urlcolor={blue!80!black}
	}
	\usepackage[a4paper, total={7in, 10in}]{geometry}
	\allowdisplaybreaks
	\newcommand{\change}[1]{{\color{red}{#1}}}
\fi
%=================================================

==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/notations.tex <==
%-----------------------------
% Notations for modeling the plant in Section of mathematical model of the system
\newcommand{\vs}{v_{\text{s}}}  % v time domain vector for stator
\newcommand{\vsd}{v_{\text{d}}} % v_d time domain for stator
\newcommand{\vsq}{v_{\text{q}}} % v_q time domain for stator
\newcommand{\is}{i_{\text{s}}}  % i vector for stator 
\newcommand{\isd}{i_{\text{d}}} % i_d  for stator
\newcommand{\isq}{i_{\text{q}}} % i_d  for stator
\newcommand{\Ls}{L_{\text{s}}}  % v vector for stator
\newcommand{\Rs}{R_{\text{s}}}  % stator resistance
\newcommand{\Kb}{K_{\text{b}}}  % back EMF constant
\newcommand{\Iqs}{I_{\text{q}}} % i_q Laplace domain for stator
\newcommand{\Vqs}{V_{\text{q}}} % v_q Laplace domain for stator
\newcommand{\Kt}{K_{\text{t}}}  
\newcommand{\Ks}{K_{\text{t}}}  % total equivalent axial stiffness

%-----------------------------
% Notations for controller gains
\newcommand{\Kp}{K_\text{p}}       
\newcommand{\Kv}{K_\text{v}}       
\newcommand{\Ki}{K_\text{i}} 
\newcommand{\Tn}{T_\text{n}}       
\newcommand{\xp}{\vc{x}^{\text{(p)}}} % Kp  
\newcommand{\xs}{\vc{x}^{\text{(s)}}} % Kv, Ki  
%-----------------------------
% Notations for performance metrics (performance is denoted by f)
% speed:
\newcommand{\fs}{f^{\text{(s)}}}                % speed performance 
\newcommand{\Fs}{F^{\text{(s)}}}                % speed vector of metrics  
\newcommand{\Ns}{N^{\text{(s)}}}                % size Fs  
\newcommand{\hs}{h^{\text{(s)}}}                % speed overshoot 
\newcommand{\hsu}{\bar{h}^{\text{(s)}}}         % speed undershoot 
\newcommand{\Ts}{T^{\text{(s)}}_{90}}           % speed settling time 
\newcommand{\es}{e^\text{(s)}}                  % speed error 
\newcommand{\esSS}{e^\text{(s)}_{\text{ss}}}    % speed steady-state error
\newcommand{\gammas}{\gamma^\text{(s)}}         % weights for speed performance
\newcommand{\alphas}{\alpha^\text{(s)}}         % trade-off weight for speed performance
% position:
\newcommand{\fp}{f^{\text{(p)}}}                % position performance 
\newcommand{\Fp}{F^{\text{(p)}}}                % position vector of metrics  
\newcommand{\Np}{N^{\text{(p)}}}                % position vector of metrics  
\newcommand{\hp}{h^{\text{(p)}}}                % position overshoot 
\newcommand{\hpu}{\bar{h}^{\text{(p)}}}         % position undershoot 
\newcommand{\Tp}{T^{\text{(p)}}_{90}}           % position settling time 
\newcommand{\ep}{e^\text{(p)}}                  % position error 
\newcommand{\epSS}{e^\text{(p)}_{\text{ss}}}    % position steady-state error
\newcommand{\epZERO}{e^\text{(p)}_0}            % position zero error
\newcommand{\gammap}{\gamma^\text{(p)}}         % weights for position performance
\newcommand{\alphap}{\alpha^\text{(p)}}         % trade-off weight for position %-----------------------------
% Miscellaneous Notations
\newcommand{\mBO}{m_\text{BO}}          % maximum BO iterations 
\newcommand{\mTRAIN}{m_\text{train}}    % number of training samples  


==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/sec_00_abstr.tex <==
\begin{abstract} % Abstract of not more than 250 words.

We propose a performance-based autotuning method for cascade control systems, where the parameters of a linear axis drive motion controller from two control loops are tuned jointly. Using Bayesian optimization as all parameters are tuned simultaneously, the method is guaranteed to converge asymptotically to the global optimum of the cost. The data-efficiency and performance of the method are studied numerically for several training configurations and compared numerically to those achieved with classical tuning methods and to the exhaustive evaluation of the cost. On the real system, the tracking performance and robustness against disturbances are compared experimentally to nominal tuning. The numerical study and the experimental data both demonstrate that the proposed automated tuning method is efficient in terms of required tuning iterations, robust to disturbances, and results in improved tracking.




%\cmm{Cascaded controller tuning is a multi-step iterative procedure, that needs to be performed routinely upon maintenance and modification of mechanical systems. An automated data-driven method for cascaded controller tuning based on Bayesian optimization is proposed. The method is tested on a linear axis drive, modelled using a combination of first principles model and system identification. A custom cost function based on performance indicators derived from system data at different candidate configurations of controller parameters is modelled by a Gaussian process.  It is further optimized by minimization of an acquisition function which serves as a sampling criterion to determine the subsequent candidate configuration for experimental trial and improvement of the cost model iteratively, until a minimum according to a termination criterion is found. This results in a data-efficient procedure, that can be easily adapted to varying loads or mechanical modifications of the system. The method is further compared to several classical methods for auto-tuning, and demonstrates higher performance according to the defined data-driven performance indicators. The influence of the training data on a cost prior on the number of iterations required to reach optimum is studied, demonstrating the efficiency of the Bayesian optimization tuning method.
%}
%In this study, a data-driven algorithm for the tuning of a cascaded controller based on Bayesian optimization is applied, that removes the need to model the system and minimizes the number of evaluations.  It is a practical optimization approach that uses Gaussian processes regression to model the performance of the system as an unknown objective function. This is done by using a probabilistic model of the cost that is updated in each iteration using the data from the system. The data is obtained by testing a set of parameters on the physical system and evaluating the cost. In order to learn fast and increase the information gained from each evaluation, the Bayesian optimization algorithm selects the next parameters to evaluate in a systematic way, for example, by maximizing information gain about the optimum. Using this process of training data and recursive sampling, the optimum values are found in a limited number of evaluations.

%The algorithm is tested on a linear motion system composed of an axis controller, motor and linear axis. The internal axis controller consists of cascaded position, speed, and current controllers connected to a motor and a load. The speed and the position controller parameters are tuned by first developing an effective cost function for the controller and testing the algorithm on the identified system model, followed by implementation on the system. The result and performance are validated with respect to existing standard tuning methods as well as the optimal value obtained from an extensive grid search. We show that Bayesian optimization is a safe, data - efficient and versatile tuning method that can be adapted to re-tune the controller for different configurations of the motion system. 

%This paper presents an automated data-driven method for the tuning of PID cascade controller gains based on Bayesian optimization. The method was used to automate the tuning of the controllers of several axis drives in a CNC grinding machine. The corresponding optimization objective is modelled using Gaussian process regression, based on data-driven performance indicators collected at different configurations of the controller gains. The posterior distribution of the modelled optimization objective is updated iteratively and an acquisition function is maximized to recommend the subsequent candidate configuration for performance evaluation until the algorithm terminates. To ensure safety, a constraint is introduced that capturies the stability requirements from system data. The algorithm was first tested in simulation, where it outperforms relay feedback autotuning and converges to the global optimum faster than other Bayesian optimization-based algorithms that keep the system within safe bounds. The implementation of the algorithm on the real system presents challenges due to additional grinding forces that lead to instabilities. A method for automatic detection of the critical gains was therefore integrated, and the optimization objective was extended by a penalty depending on the proximity to critical gains of the current candidate points. The proposed method for automated and standardized tuning procedure achieves the same grinding performance as nominal tuning.
	
	
% ~ Rewrite 
%Cascaded controller tuning is a multi-step iterative procedure, that needs to be performed routinely upon maintenance and modification of mechanical systems. An automated data-driven method for cascaded controller tuning based on Bayesian optimization is proposed. The method is tested on a linear axis drive, modelled using a combination of first principles model and system identification. A custom cost function based on performance indicators derived from system data at different candidate configurations of controller parameters is modelled by a Gaussian process.  It is further optimized by minimization of an acquisition function which serves as a sampling criterion to determine the subsequent candidate configuration for experimental trial and improvement of the cost model iteratively, until a minimum according to a termination criterion is found. This results in a data-efficient procedure, that can be easily adapted to varying loads or mechanical modifications of the system. The method is further compared to several classical methods for auto-tuning, and demonstrates higher performance according to the defined data-driven performance indicators. The influence of the training data on a cost prior on the number of iterations required to reach optimum is studied, demonstrating the efficiency of the Bayesian optimization tuning method.
%--------------------------------------------------------------------------------------------------
%In this study, a data-driven algorithm for the tuning of a cascaded controller based on Bayesian optimization is applied, that removes the need to model the system and minimizes the number of evaluations.  It is a practical optimization approach that uses Gaussian processes regression to model the performance of the system as an unknown objective function. This is done by using a probabilistic model of the cost that is updated in each iteration using the data from the system. The data is obtained by testing a set of parameters on the physical system and evaluating the cost. In order to learn fast and increase the information gained from each evaluation, the Bayesian optimization algorithm selects the next parameters to evaluate in a systematic way, for example, by maximizing information gain about the optimum. Using this process of training data and recursive sampling, the optimum values are found in a limited number of evaluations.

%The algorithm is tested on a linear motion system composed of an axis controller, motor and linear axis. The internal axis controller consists of cascaded position, speed, and current controllers connected to a motor and a load. The speed and the position controller parameters are tuned by first developing an effective cost function for the controller and testing the algorithm on the identified system model, followed by implementation on the system. The result and performance are validated with respect to existing standard tuning methods as well as the optimal value obtained from an extensive grid search. We show that Bayesian optimization is a safe, data - efficient and versatile tuning method that can be adapted to re-tune the controller for different configurations of the motion system. 
\end{abstract}




==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/sec_01_intro.tex <==
\section{Introduction}

Routine maintenance of mechatronic systems requires the periodic tuning of PID controllers of linear or rotational drives to counter the gradual decline of performance due to the increase of friction, loosening of mechanical components, or wear. The corresponding PI and PID gains are often set to conservative values to ensure operation for a broad range of loads or mechanical properties, focusing on disturbance rejection.
While gain autotuning is in principle possible, existing off-the-shelf autotuning routines often interfere with safety mechanisms in manufacturing systems and are often avoided.

In classical model-based controller design, a model of the plant is derived from first-principle methods or identified using experimental data, and then a controller is designed based on this model \cite{feedbackSys}. For example, symmetric optimum tuning \cite{kessler58}, and its extensions \cite{Preitl99} provide relations between the controller gains and the achievable performance in terms of settling time, phase margin, overshoot, and other relevant metrics. Model-based methods are data-efficient and tuning can be achieved with relatively few iterations. For cascade control systems however, multiple cycles of tuning might be required, and the achieved values of the controller parameters are mostly on the conservative side. Whenever first-principle methods cannot be used, optimization problems arise in obtaining the final controller, both in computation of the model and the controller, through the minimization of prediction error criterion, or criteria based on controller stability and transient smoothness. A controller that best fits the frequency response of the optimal controller is obtained by optimization or order reduction techniques \cite{Karimi2017}. Performance-based objective functions based on calculating the error signal between the system output and the input reference signal such as e. g. Integral Square Error (ISE), Integral Absolute Error (IAE) or Integral Time Absolute Error (ITAE), are often minimized to tune controller parameters using genetic algorithms \cite{daSilva2000} or Particle Swarm Optimization \cite{Qi2019}, and often require a large number of evaluations to ensure that a global optimum is found. Standard methods, such as the Ziegler-Nichols rule \cite{ziegler1942optimum} or relay tuning with additional heuristics \cite{hang2002relay, Kumar2015} are routinely used for the tuning in practice and will be used here as benchmark results in simulation.

Various data-driven methods for controller design have been proposed, e.g. virtual reference feedback tuning (VRFT) \cite{Campi2002, Campi2006}, data-driven inversion-based control \cite{Novara2018}, direct learning of linear parameter varying (LPV) controllers from data \cite{Formentin2016}, data-driven controller tuning in mixed-sensitivity loop-shaping framework. Data-driven tuning has been explored in an iterative learning approach in \cite{Prochazka2005}, and also combined with a learned process model in \cite{Radac2014}. While they find application, the methods often work under assumptions of linearity or time invariance for the plant or the closed loop system. Iterative learning approaches might require multiple iterations or interventions through external probing signals or specially designed references. Data-driven methods often do not allow for constraints in the input and output variables, and the choice of reference models is also dependent on prior knowledge of the system \cite{Bazanella2014}.

Bayesian optimization (BO) is used for hyperparameter tuning in high-dimensional machine learning models, but it has also gained attention in engineering and has been applied e.g., to control of quadrotors combined with learned dynamics \cite{Tomlin}, optimization of process set-up parameters \cite{Maier2019, Maier_2020gr,}, and  collision avoidance \cite{Andersson2016}. Bayesian data-driven approaches have been also proposed for the tuning of PID controllers and of nonlinear systems \cite{BayesOpt1, BayesOpt2,khosravi2019controller,khosravi2019machine}. These approaches are particularly interesting because of the inherent data-efficiency and flexibility of the Bayesian optimization (BO) method. BO in controller tuning, where stability is guaranteed through safe exploration, has been proposed in \cite{BayesOpt1}, and applied to robotic applications \cite{BayesOpt5}, and in process systems \cite{khosravi2019controller}. Constraint BO tuning is proposed in \cite{SafetyBO2020}.

We propose a performance-based BO approach for autotuning of the cascaded controller parameters of a linear axis drive where the controller parameters of interest are tuned simultaneously. The tuning problem is formulated as an optimization where the controller parameters are the variables that ensure a minimum in the cost defined through a weighted sum of performance metrics extracted from encoder signals. In this work, we restrict the range of the optimization variables to a limited set where the system is stable. We focus on overshoot and setpoint tracking errors as performance metrics, and demonstrate that the method ensures disturbance rejection as in the nominal tuning methods. Simultaneous tuning of all parameters eliminates the need for successive tuning trials for each control loop, while the method is guaranteed to converge to a global optimum due to the properties of Bayesian optimization. The rest of this paper is organized as follows: Section \ref{sec:problem_statement} introduces the general problem of performance-driven cascaded controller tuning in linear axis drives. Section \ref{sec:system_model} presents the plant model derived from first principles and system identification techniques. Section \ref{sec:num_results} introduces the performance-based approach with numerical results comparing the proposed tuning method with standard tuning methods, also with an evaluation of the performance metrics on a grid. Experimental validation is reported in Section \ref{sec:experimental}.

%In section \ref{sec:GP_BO}, we review the required preliminaries for Gaussian processes and Bayesian optimization.

%We apply it in simulation and on a linear motion system with a cascade controller and compare the achieved performance with standard tuning methods. 

==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/sec_02_probl.tex <==
%\section{Mathematical Notations} \label{sec:Not}
%In this paper, the set of natural numbers, the set of integers, the set of real numbers, the $n$-dimensional Euclidean real space and the set of $n$ by $m$ matrices are denoted by $\Nbb$, $\Zbb$, $\Rbb$, $\Rbb^n$ and $\Rbb^{n\times m}$ respectively. The identity matrix and zero matrix in $\Rbb^{n\times n}$ are denoted by  $\eye_n$ and  $\zeromx_{n}$, respectively, and the zero vector and the all-one vector in  $\Rbb^n$ are denoted by $\zero_n$ and $\one_n$, respectively. When the dimensions of these matrices or vectors are clear from the context, we drop the subscript. The Gaussian distribution with mean $\mu$ and covariance $\Sigma$ is denoted by $\Ncal(\mu,\Sigma)$. \cmr{[see comment]}
%Mohammad: For now, we should keep the notations and try to distribute it through the paper.

\section{Performance-Based Tuning}
%Here we investigate the problem of performance-based data-driven tuning of a multi-loop cascade controller.
The system of interest is a ball-screw drive, a positioning mechanism used routinely in machining systems. Notable applications of such systems are in the semiconductor industry, in biomedical engineering, and in the photonics and solar technologies. The ball-screw drive components are shown in Figure \ref{mfig:structure}. The AC motor is connected via a coupling joint to a ball-screw shaft fixed to a supporting frame. 
\label{sec:problem_statement}
\begin{figure}[t]
	\centering
	\includegraphics[width = 0.37\textwidth]{Figs/autotuning_labels1.pdf}%    
	\caption{The structure of ball-screw system:
		\textcircled{\small{1}} DC motor, \textcircled{\small{2}} coupling joint, \textcircled{\small{3}} ball-screw interface, 
		\textcircled{\small{4}} nut, 
		\textcircled{\small{5}} ball-screw shaft, \textcircled{\small{6}} guideway and 
		\textcircled{\small{7}} table (load), following \cite{altintas2011machine}.
	}
	\label{mfig:structure}
	\vspace{-4mm}
\end{figure}
The shaft carries a nut which converts the rotational motion of the shaft linear motion of the nut through a screw-nut interface. 
The system is equipped with encoders for measuring the nut position, the rotational speed of the motor and the linear speed of the ball-screw shaft, and a sensor for measuring the motor current. The set voltage of the motor is controlled  through a motor drive and a programming logic controller (PLC). Typically, the motor rotates the shaft, the nut moves from initial to final position, remains there for some time and returns to the initial position. The position and speed of the nut are controlled such that they follow designed ideal reference trajectories (see Figure \ref{fig:perf_metrics}).

 We introduce a performance metric indicating the quality of tracking, calculated from the position and speed error signals.  The error signals and the performance metric are functions of the vector of parameters describing the controller, denoted here by $\vc{x}$. Let the performance function be $f: \Xcal\to\Rbb$ where $\Xcal$ is the space of admissible controller parameters. % and $\Rbb$ is the set of real numbers. 
With respect to controller parameters, $\vc{x}$, the performance function does not have a tractable closed-form expression, even when the dynamics of system are known. 
For a given $\vc{x} \in \Xcal$, the value of the performance metric $f(\vc{x})$  has a {\em black-box oracle} form, and can be obtained experimentally from the position and speed tracking error signals $\ep_m$ and $\es_m$, for controller parameters set to $\vc{x}$. 
%For a given $\vc{x} \in \Xcal$, the value $f(\vc{x})$ can be obtained purely in a data-driven way by performing an experiment with parameters of controllers being set to $\vc{x}$, and then calculating the performance metric based on the tracking error signals.  
%The black-box oracle form of the performance function is unknown, due to the dynamics of system, and to the complexity of its dependency to the parameters. 
%Though, by performing a system identification procedure one may partially address the latter issue, the former concern still exists. 
%-----
%The ideal trajectories for position and for speed are indicated by the red curves in Figure \ref{fig:perf_metrics}. The performance of the controller or the appropriateness of chosen corresponding parameters can be described in terms of the quality of tracking the ideal trajectories. We introduce several quantitative metrics derived from the data focused in quantifying the tracking performance, shown in Figure \ref{fig:perf_metrics}. The performance metrics in accordance with position reference tracking are the overshoot, $\hp$, the 90\% settling time of the position step response, $\Tp$, the tracking error in position quantified by its infinity norm $\|\ep\|_{\infty}$. Similarly, the performance metrics for tracking speed reference trajectory are the overshoot of speed in the departure phase, $\hs$, the overshoot of the speed in returning phase, $\bar{h}^{\text{(s)}}$, the 90\% settling time of the speed step response, $\Ts$, the speed tracking error quantified by its infinity norm, $\|\es\|_{\infty}$, the steady-state error, $\hs_{\text{ss}}$, and the integral of the time-weighted absolute value of the error of the speed response, $\es_{\text{ITAE}}$. A more detailed discussion on the performance metrics follows in Section \ref{sec:performance_based_tuning_methods}.
%Each of these metrics reflects a feature of tracking the reference trajectories. The combination of the features in this work is done by a weighted sum where each of the weights depends on the scale and the importance of corresponding metric and feature. 
%------
%Once we introduce the data-driven performance criteria as a function of the vector of parameters describing the controller, denoted by $\vc{x}$, we have the means to find the parameters providing optimal performance.  
%Let $f: \Xcal\to\Rbb$ denote the performance metrics where $\Xcal$ is the space of admissible parameters. 
%The dependency of $f$ to $\vc{x}$ has {\em black-box oracle} form even when the dynamics of system is completely known. 
%More precisely, the closed-form expression of $f$ is not known and not accessible. For a given $\vc{x} \in \Xcal$, the value $f(\vc{x})$ can be obtained only by performing an experiment with parameters being set to $\vc{x}$, and then calculating the performance metrics based on the observed position and speed trajectories. 
%The black-box oracle form of the combined performance metrics is unknown, due to the dynamics of system, and to the complexity of its dependency to the parameters. 
%Though, by performing a system identification procedure one may partially address the latter issue, the former concern still exists. 
%----
We propose tuning the controller parameters based on a data-driven procedure of performing a sequence of experiments, collecting data, assessing the corresponding performance, and utilizing Bayesian optimization as a  black-box optimization technique for deriving optimal vector of controller gains (see Figure \ref{fig:scheme}). 
%More precisely, let the $m^{\text{\tiny{th}}}$ round of experiment be performed in time interval  $I_m:=[t^{\text{(i)}}_m,t^{\text{(f)}}_m]$ 
%with vector of controller gains being set to $\vc{x}_m\in\Xcal$. 
%Also, let $\ep_m:I_m\to\Rbb$ and $\es_m:I_m\to\Rbb$ be respectively the corresponding error signals for position tracking and speed tracking. 
%Once the experiment is performed and signals $\ep_m$ and $\es_m$ are measured, we can calculate the resulting tracking performance metric, denoted by $y_m =f(\vc{x}_m)+w_m$ where $f(\vc{x}_m)$ is the true performance and $w_m$ is the uncertainty due to noise in measurements. 
The estimated performance at each trial is provided to the performance-based tuning unit which is essentially a Bayesian optimization module. This unit models the performance metric using {\em Gaussian process regression} (GPR) \cite{GPR}, and finds the optimal parameters based on a suitable Bayesian optimization algorithm as {\em Gaussian process lower confidence bound} (GP-LCB) ~\cite{srinivas2012information}. %The overall tuning scheme is shown in Figure \ref{fig:scheme}.

\begin{figure}[t]
\centering
\includegraphics[width = 0.37\textwidth]{Figs/BlockDiagram_BO_in_loop6.pdf}%    
\caption{The performance-based controller tuning scheme.}
\label{fig:scheme}
\vspace{-4mm}
\end{figure}

The proposed tuning approach is  performance-based, model-free and data-driven. One of the main advantages of utilizing Bayesian optimization is its potential in explicitly modeling noise which is automatically considered in the uncertainty evaluation without skewing the result~\cite{srinivas2012information}. The simultaneous optimization of all parameters guarantees convergence to the global optimum performance, following from the properties of Bayesian optimization, at the cost of more iterations compared to classical approaches. 
\vspace{-0.5cm}
%This can be achieved only through iterative improvement, therefore potentially more iterations than using classical deterministic approaches are required to find optimal parameters. 
%This can be achieved only through iterative improvement with potentially more iterations than usual classical deterministic approaches.
%A way to reduce the iterations during tuning is to have a comprehensive prior model of the performance metric. We explore the trade-off between the number of optimization iterations and the required trials for collection of training data for the prior model in detail in Section \ref{sec: BO_sim}.



==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/sec_03_preli.tex <==
\section{Gaussian Processes and Bayesian Optimization} \label{sec:GP_BO}
%Bayesian optimization is a data-driven approach for solving optimization problems where the objective function is unknown and available in form of a noisy {\em oracle}. 
%BO samples and learns the objective function efficiently online by querying the oracle for different candidate configurations of inputs. BO uses Gaussian process regression (GPR) iteratively to build a surrogate for the objective function and quantify the associated uncertainty~\cite{BayesOpt4} for all possible configurations. In each iteration, the data is used for deciding on the next evaluation point based on an acquisition function. 
%The new information, the result of queried oracle on the new evaluation point, is combined with the prior knowledge using Gaussian process regression to estimate the objective function, and to find its minimum~\cite{BayesOpt4}, corresponding to the optimal input configuration. 
\subsection{Gaussian Processes}
\label{GP}
A Gaussian process (GP) is a collection of random variables where each of its finite subsets is jointly Gaussian \cite{GPR}. 
The GP is uniquely characterized by the mean function, $\mu:\Xcal \to \Rbb$, and the  covariance/kernel function, $k:\Xcal\times\Xcal\to \Rbb$, where $\Xcal$ is the set of location indices.
The GP is denoted by $\GP{\mu}{k}$ %or $\GP{\mu(\cdot)}{k(\cdot,\cdot)}$
, $\Xcal$ is a subset of $\Rbb^d$ and the kernel is the {\em square exponential} kernel
\begin{equation}
k_{\text{SE}}(\vc{x},\vc{x}') \!=\!
\sigma_{f}^2\exp{\bigg{(}\!\!-\!\frac{1}{2}(\vc{x}\!-\! \vc{x}')^{\tr}\mathrm{L}^{-1}(\vc{x}\!-\!\vc{x}')\!\bigg{)}},
\end{equation}
for any $\vc{x},\vc{x}'$ in $\Xcal$ where $\sigma_f$ and $\mathrm{L}$ 
% and $\sigma_n$ 
are the hyperparameters of the kernel, respectively referred as {\em length scale matrix} and {\em flatness parameter}. % and {\em noise variance}, and $\delta_{\vc{x},\vc{x}'}$ is {\em Kronecker delta} function, i.e.,  $\delta_{\vc{x},\vc{x}'}=1$, if $\vc{x}=\vc{x}'$ and $\delta_{\vc{x},\vc{x}'} = 0$, otherwise. 

Gaussian processes provide flexible models for Bayesian learning by introducing prior distributions  over the space of functions defined on $\Xcal$.
Due to the favorable properties of the Gaussian distributions, the marginal and the conditional mean and variance can be computed on any finite set of locations in a closed form. 
%Subsequently, a probabilistic  non-parametric regression  method can be developed \cite{GPR}.
%More precisely, let $f:\Xcal\to\Rbb$ be an unknown function, $\GP{\mu}{k}$ be the prior distribution for estimating $f$, and noisy measurements at locations $\vcc{x} := \begin{bmatrix}\vc{x}_1& \vc{x}_2 &\ldots &\vc{x}_m\end{bmatrix}$ be given as  $\vcc{y} := \begin{bmatrix}\vc{y}_1& \vc{y}_2 &\dots& \vc{y}_m\end{bmatrix}^\tr\in\Rbb^m$. 
Let $f:\Xcal\to\Rbb$ be an unknown function, $\GP{0}{k}$ be the prior distribution for estimating $f$, and noisy measurements at locations $\vc{x}_1,\ldots,\vc{x}_m$ be respectively given as  $\vc{y}_1,\dots,\vc{y}_m$. 
In other words, we know that $f\sim \GP{0}{k}$ and  $\vc{y}_i=f(\vc{x}_i)+w_i$, for $i=1,\ldots,m$, where $w_i$ is the measurement noise with zero mean Gaussian distribution $\Ncal(0,\sigma_w^2)$. 
Since there is no additional information about the latent function $f$, we can set the mean of the GP prior to zero. 
Let $\vc{x}\in\Xcal$ be a new location where the corresponding measurement is not provided. 
Since the joint distribution of the measurements data is Gaussian with a given mean and a given covariance, one can predict the value of measurement at the new location $\vc{x}$ using {\em Bayes rule}. 
First, we define $\mx{X}_m$ and $\vc{y}_m$ respectively as $\mx{X}_m:= [\vc{x}_1,\vc{x}_2,\ldots,\vc{x}_m]\in\Rbb^{n\times m}$ and $\vc{y}_m := [y_1,y_2,\ldots,y_m]^\tr\in\Rbb^m$.
Also, we define the Gram matrix $\mathrm{K}_{{\mx{X}_m\mx{X}_m}}\in\Rbb^{m\times m}$ such that its  element at the $i^{\text{\tiny{th}}}$ row and the $j^{\text{\tiny{th}}}$ column is given by $k(\vc{x}_i,\vc{x}_j)$. 
Consequently, due to $f\sim \GP{0}{k}$, we know that 
$\vc{y}_m \sim \Ncal\big{(}\zero,\mx{K}_{\mx{X}_m\mx{X}_m}+\sigma^2_w\eye\big{)}$, where $\eye$ denotes the identity matrix.
%\begin{equation}
%     \mathrm{y} \sim \mathcal{N}\bigg{(}0,\mathrm{K}_{\mathrm{xx}}+\sigma^2_n\mathbb{I}\bigg{)} \,.
%\end{equation}  
The joint distribution of the training data $\{(\vc{x}_i,y_i)\}_{i=1}^m$ with the new data point $(\vc{x},y_\vc{x})$, where  $y_\vc{x} := f(\vc{x})$ is the unknown label for location $\vc{x}$, can be calculated as 
\begin{equation}
    \begin{bmatrix}
    \vc{y}_m\\y_\vc{x}
    \end{bmatrix} \sim \mathcal{N}\bigg{(}0,\begin{bmatrix} \mx{K}_{\mx{X}_m\mx{X}_m} + \sigma^2_w\eye & \vc{k}_{\vc{x}\mx{X}_m}^\tr \\ \vc{k}_{\vc{x}\mx{X}_m} & k_{\vc{x}\vc{x}} \end{bmatrix}\bigg{)}  \,,
\end{equation} 
where $\mathrm{k}_{\vc{x}\mx{X}_m}\in\Rbb^m$ is the vector such that its $i^{\text{\tiny{th}}}$ element is given by the kernel as $k(\vc{x},\vc{x}_i)$, for any $i=1,\ldots,m$, and $ k_{\vc{x}\vc{x}}:=k(\vc{x},\vc{x})$. The posterior distribution of $y_{\vc{x}}|\mx{X}_m,\vc{y}_m$ is a Gaussian distribution as
\begin{equation}
    y_{\vc{x}} | \mx{X}_m,\vc{y}_m \sim \mathcal{N}(\mu_m(\vc{x}),\sigma_m(\vc{x})) \,,
\end{equation}
where the mean of prediction, $\mu_m(\vc{x})$, and the corresponding covariance, $\sigma_m(\vc{x})$, are given as 
\begin{align}
\mu_m(\vc{x}) &:= \vc{k}_{\vc{x}\mx{X}_m}^\tr\big{(}\mx{K}_{\mx{X}_m\mx{X}_m}+\sigma^2_w\eye\big{)}^{-1}\vc{y}_m,
\label{eqn:mu}\\
\sigma_m(\vc{x}) &:= k_{\vc{x}\vc{x}} - \mathrm{k}_{\vc{x}\mx{X}_m}^\tr\big{(}\mathrm{K}_{\mx{X}_m\mx{X}_m}+\sigma^2_w\eye\big{)}^{-1}\vc{k}_{\vc{x}\mx{X}_m}. \label{eqn:sigma}
\end{align}
The posterior mean $\mu_m(\vc{x})$ is a nonlinear function predicting the value of $f$ at location $\vc{x}$ with an uncertainty  described by $\sigma_m(\vc{x})$. Accordingly, this is a nonlinear non-parametric regression method called {\em Gaussian process regression} (GPR).
%The GPR depends on hyperparameters such as .
The hyperparameters of the kernel $\sigma_f$, $\mx{L}$ and $\sigma_w$ collected in a vector $\theta\in\Theta$ can be estimated by minimizing the negative log marginal log-likelihood of the joint distribution of the training data,
\begin{equation}\label{eqn:min_nlml}
\hat{\theta}:= 
\argminOp_{\theta\in\Theta}\ -\log p(\mathrm{y}_m|\mx{X}_m,\theta) \, ,
\end{equation}
where $ p(\mathrm{y}_m|\mx{X}_m,\theta)$ is the probability density function of the labels or measurements acquired at locations $\{\vc{x}_i\}_{i=1}^m$. 
%________________________________
%________________________________
\subsection{Bayesian Optimization Algorithm}
The goal of Bayesian optimization is to find efficiently a solution for the problem
\begin{equation}\label{eqn:x_star_argmin_f}
\vc{x}^* = \argminOp_{\vc{x}\in\Xcal}\ f(\vc{x}) \,,
\end{equation} 
where $f:\Xcal\to \Rbb^n$ is an unknown function that is expensive to evaluate, available only as a noisy {\em oracle}. In the optimization \eqref{eqn:x_star_argmin_f},  $\vc{x}$ can be a vector of design parameters or decision variables. Similarly, $f$ can be a user-defined cost function or a specific designed performance indicator.

In Bayesian optimization, the information about the unknown objective is collected by efficient on-line sampling and querying the oracle, and subsequently, learning the unknown function and deriving the global optimal solution iteratively. %More precisely, a set of sampling points is generated sequentially for which the oracle is queried.
For any $m\in\Nbb$, let $\vc{x}_m\in\Xcal$ and $y_m\in\Rbb$ denote respectively the $m^{\text{\tiny{th}}}$ sampling point and the corresponding value returned by the oracle.
 Since the oracle is noisy, we have $y_m = f(x_m)+w_m$, where $w_m$ is the evaluation noise of oracle.
 In each sampling iteration $m\in \Nbb$, a surrogate function is learned for the unknown objective function using Gaussian process regression and the associated uncertainty is quantified, using \eqref{eqn:mu} and \eqref{eqn:sigma}.
 %At iteration $m\in \Nbb$, given noisy measurements  $y_1,\dots,y_m$ respectively for sampling locations $\vc{x}_1,\ldots,\vc{x}_m$,
%using Gaussian process regression, one can obtain the posterior distribution and also,  $\mu_m$ and $\sigma_m$ as in \eqref{eqn:mu} and \eqref{eqn:sigma}.
Accordingly, $\mu_m$ is the surrogate function and $\sigma_m$ quantifies the corresponding uncertainty in the prediction of the value of objective function on the future sampling point.
The next candidate evaluation point $\vc{x}_{m+1}$
is determined based on a sampling criterion called {\em acquisition function}. 
Commonly used acquisition functions include \textit{entropy search}, \textit{expected improvement}, \textit{upper confidence bound (UCB)}, etc~\cite{BayesOpt4}.
The acquisition function provides a trade-off between exploitation and exploration.  %It can explore regions of the domain with maximum information and highest prediction uncertainty, exploit the point with the lowest predicted cost or select new locations according to a combination of these two objectives~\cite{srinivas2012information}. 
Here we use the {\em lower confidence bound} (LCB) of the predicted objective function~\cite{srinivas2012information}, defined as 
\begin{equation}\label{eqn:GP_LCB}
\vc{x}_{m+1}=\argminOp_{\vc{x} \in \Xcal}\ \mu_{m}(\vc{x})-\beta_{m}\sigma_{m}(\vc{x}) \, ,
\end{equation}
where
$\beta_{m}$ is a constant specifying the considered confidence bound around the mean function $\mu_m$. The LCB acquisition function selects points $\boldsymbol{x}$ with large uncertainty $\sigma_{m}$ and with low cost prediction $\mu_{m}$. %It implicitly negotiates the exploration - exploitation trade-off.
A natural interpretation of this sampling rule is that it greedily selects points $\vc{x}$ where $f(\vc{x})$ could be lower than the current minimum and upper bounds the function by the current minimum \cite{srinivas2012information}.

Let $m^*$ be the index of sampling point with minimum observed cost amongst $\vc{x}_1,\ldots,\vc{x}_m$, i.e., 
\begin{equation}\label{eqn:mstar}
m^* = \argmin_{i\in\{1,2,\ldots,m\}}y_i.    
\end{equation}
While it is guaranteed that as $m$ goes to infinity, the uncertainty is reduced and the best observed point, $\vc{x}_{m^*}$, converges to the $\vc{x}^*$, we need to introduce a finite-time practical stopping criterion ~\cite{srinivas2012information}. 
%The suitable criteria are case-dependent and need to be decided based on the underlying application and the system specifications. 
Since the primary goal is to reduce the number of evaluations, the stopping condition used here is limiting the number of iterations to be less than a predefined maximum number, denoted by $\mBO$. %An additional stopping criterion is introduced to reduce further the number of iterations.
When sampling occurs repeatedly around the current minimum, the algorithm is terminated after three successive iterations. The stopping criteria are flexible and can be determined according to the specific applications of the tuning algorithm.

==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/sec_04_sys.tex <==
\section{System Structure and Model} \label{sec:system_model}
%We derive a parametric, first principles model of the system and introduce the controller structure.
%We set the parameters of the model either from the provided data-sheets, or estimate them from experimental data. The derived model will be used later for numerical verification of our controller tuning method.

%____________________________________________________
\subsection{Mathematical Model of System} \label{sec_plant_math}
%To obtain a mathematical representation of the plant, both the electrical and mechanical parts of the system have to be modelled. We first derive the dynamics of the AC motor according to its equivalent electrical circuit and the mechanical equations of motion. 

The motor deriving the ball-screw system is a {\em permanent-magnet synchronous motor}, with a  permanent magnet on the rotor providing the exciting field. Let $\Rs$ and $\Ls$ respectively denote the resistance and the inductance of the stator.
From Kirchhoff's voltage law and the back electromotive force (EMF) which comes from Faraday's law of induction, in the dq-frame we have
\begin{equation*}
\label{eqn:v_dq_dynamics_1}
\!\!\!\!\!\!\!
\begin{split}
\vsd(t) &= 
\Ls \frac{\mathrm{d}}{\mathrm{d}t}\isd(t)
+ \Rs\isd(t) - \Ls\omega_{\text{m}}(t)\isq(t),
\\
\vsq(t) &= \Ls \frac{\mathrm{d}}{\mathrm{d}t}\isq(t)+ \Rs\isq(t) + \Ls\omega_{\text{m}}(t)\isd(t) + \Kb\omega_{\text{m}}(t),\\ 
\end{split}\!\!\!
\end{equation*}
where $[\vsd \ \vsq]^\tr$ and $[\isd\ \isq]^\tr$ are respectively the vectors of stator voltage and stator current in dq-coordinates, 
$\Kb$ is the back EMF constant and  $\omega_{\text{m}}$ is the angular velocity of the motor and shaft.
The d-component of the current, $\isd$, only influences the component of the magnetic field in the direction of the rotor axis and does not contribute to the torque generation. 
To minimize losses a PID-controller regulates $\vsd(t)$ to compensate the voltage induced by $\isq$ and ensures that $\isd = 0$ at all times.
Consequently, the resulting dynamics of motor is 
\begin{equation}\label{eqn:v_dq_dynamics_2}
\begin{split}
\vsd(t) &= - \Ls \omega_{\text{m}}(t)\isq(t) ,
\\
\vsq(t) &= \Ls \frac{\mathrm{d}}{\mathrm{d}t}\isq(t)+ \Rs\isq(t) + \Kb\omega_{\text{m}}(t).
\end{split}
\end{equation}
The motor develops an electromagnetic torque $\tau_{\text{m}} = \Kt \isq$ proportional to the stator q-component of current.
%By tacking the Laplace transform, 
One can obtain the transfer function of motor as 
\begin{equation}\label{eqn:M(s)}
M(s) 
\!:=\! 
\frac{\Omega_{\text{m}}(s)}{\Vqs(s)}  
\!=\! 
K_{\text{t}}
\ \!
\big{(}K_{\text{t}}K_{\text{b}} \!+\!(\Ls s \!+\! \Rs)\Big(\frac{T_{\text{m}}(s)}{\Omega_{\text{m}}(s)}\Big)\big{)}^{-1}
\!\!,
\end{equation}
where $\Omega_{\text{m}}$, $\Vqs$ and $T_{\text{m}}$ are the Laplace transform of $\omega_{\text{m}}$, $\vsq$ and $\tau_{\text{m}}$, respectively.
%As shown in Figure \ref{mfig:structure}, the motor is connected to the ball-screw drive via flexible couplings and the drive is constrained to the machine base by means of fixed rotary bearings \cite{altintas2011machine,AxisModelling}.
The main limitation on the accuracy of the linear position is due to the {\em first axial mode} of the ball-screw system \cite{AxisModelling}, which is determined by the flexibility characteristics of the translating components.
This includes the inherent stiffness of the ball-screw and the bearings as well as the interactions between the carriage table, the nut and the ball-screw \cite{altintas2011machine,2DOFControl1,AxisModelling}.
The first axial dynamics of the ball-screw servo drive can be modelled using a simplified two degree of freedom  mass-spring-damper system \cite{altintas2011machine}.  
If we let $J_{\text{m}}$, $B_{\text{m}}$ and $\theta_{\text{m}}$ be inertia, damping coefficient and angular displacement of the motor, and $J_{\text{l}}$, $B_{l}$, $\theta_{\text{l}}$ and $\omega_{\text{l}}$ 
the corresponding quantities of the load, a torque balance leads to
\begin{equation}\label{eqn:omega_ml}
\begin{split}
&\!\! J_{\text{m}} \frac{\mathrm{d}\omega_{\text{m}}}{\text{d}t} + B_{\text{m}} \omega_{\text{m}} + B_{\text{ml}} (\omega_{\text{m}} - \omega_{\text{\text{l}}}) + K_{\text{s}} (\theta_{\text{m}}- \theta_{\text{l}}) = \tau_{\text{m}},\! \\&
\!\! J_{\text{l}}\ \! \frac{\text{d}\omega_{\text{l}}}{\text{d}t} + B_{\text{l}}\ \!\omega_{\text{l}} - B_{\text{ml}} (\omega_{\text{m}}- \omega_{\text{\text{l}}}) - K_{\text{s}} (\theta_{\text{m}} - \theta_{\text{l}}) = \tau_{\text{l}},\!
\end{split} 
\end{equation}
where $K_{\text{s}}$ is the total equivalent axial stiffness, $\tau_{\text{l}}$ is the torque disturbance of the load and $B_{\text{ml}}$ is the damping coefficient between the coupling and the guides. 
As $B_{\text{l}}$ has a negligible impact on resonance, one can set $B_{\text{l}}=0$ \cite{altintas2011machine}. 
Taking the Laplace transform leads to
\begin{equation}\label{eqn:Transfer_theta_tau}
\begin{bmatrix}
\Theta_{\text{m}}(s)\\\Theta_{\text{l}}(s)
\end{bmatrix}
=
\mathrm{H}(s)^{-1}
\begin{bmatrix}
T_{\text{m}}(s) \\ T_{\text{l}}(s)
\end{bmatrix},
\end{equation}
where capital letters denote the Laplace transform of the corresponding quantities and  $\mathrm{H}(s)$ is defined as
\begin{equation*}\label{eqn:H(s)}
\mathrm{H}(s)\! := \! \begin{bmatrix}
\!J_{\text{m}}s^2
\!+\!
(B_{\text{m}}\!+\!B_{\text{ml}})s
\!+\! 
K_{\text{s}}
& 
-B_{\text{ml}}s
-K_{\text{s}}
\\
- B_{\text{ml}}s - K_{\text{s}}
&\!\!\!\!\!\!\!
J_{\text{l}}s^2
\!+\!
(B_{\text{l}}\!+\!B_{\text{ml}})s
\!+\! 
K_{\text{s}}\!
\end{bmatrix}\!.
\end{equation*}
%\begin{equation}\label{eqn:H(s)}
%\begin{split} &\mathrm{H}(s) := \\  
%&\begin{bmatrix} J_{\text{m}}s^2 + (B_{\text{m}}+B_{\text{ml}})s +
% K_{\text{s}} & -B_{\text{ml}}s -K_{\text{s}}\\ - B_{\text{ml}}s - K_{\text{s}}
% & J_{\text{l}}s^2 + (B_{\text{l}}+B_{\text{ml}})s +  K_{\text{s}} \end{bmatrix}.\end{split}\end{equation}
% ? Isn’t the load torque the main source of disturbance?
% I don’t think you need to set anything to zero, just derive the TF from motor torque to the angular velocities.
Due to the structure of the linear axial system, the torque disturbance of the load comparing to motor torque is negligible.
Therefore, to derive the transfer function from motor torque to the angular velocity, we set $T_{\text{l}}(s) =0$.
Let $D(s)$ denote the determinant of $\mathrm{H}(s)$. To obtain the transfer functions relating the motor to the angular velocities, we define transfer functions 
%\begin{align}{F_1(s)} &:= \frac{\Omega_{\text{m}}(s)}{T_{\text{m}}(s)} = \frac{J_{\text{l}} s^2 + B_{\text{ml}} s + K_{\text{s}}}{D(s)},\label{eqn:T1}\\{F_2(s)} &:= \frac{\Omega_{\mathrm{l}}(s)}{T_{\text{m}}(s)} = \frac{B_{\text{ml}} s + K_{\text{s}}}{D(s)},\label{eqn:T2}\end{align}
$F_1(s) := 
\Omega_{\text{m}}(s)/T_{\text{m}}(s) = (J_{\text{l}} s^2 + B_{\text{ml}} s + K_{\text{s}})/D(s)$, 
$F_2(s):= \Omega_{\mathrm{l}}(s)/T_{\text{m}}(s) = (B_{\text{ml}} s + K_{\text{s}})/D(s)$,
and subsequently,
\begin{align}
{F_3(s)} &:= \frac{\Omega_{\mathrm{l}}(s)}{\Omega_{\text{m}}(s)} = \frac{F_2(s)}{F_1(s)} = 
\frac{B_{\text{ml}} s + K_{\text{s}}}{J_{\text{l}} s^2 + B_{\text{ml}} s + K_{\text{s}}}. \label{eqn:T3}
\end{align}
%where $\Omega_{\mathrm{l}}$ is the Laplace transform of $\omega_{\text{l}}$. Now, regarding the 
Combining with \eqref{eqn:M(s)} leads to the
transfer function between the voltage applied to the armature and  rotational velocity of the load \cite{2DOFControl1}
\begin{equation} \label{eqn:G(s)_eq1}
\begin{split}
G(s) &:= \frac{\Omega_{\text{l}}(s)}{\Vqs(s)} = \frac{\Omega_{\text{m}}(s)}{\Vqs(s)} \frac{\Omega_{\text{l}}(s)}{\Omega_{\text{m}}(s)}= M(s)\ {F_3(s)}
\\&=
K_{\text{t}}
\ \!
\big{(}K_{\text{t}}K_{\text{b}} \!+\!(\Ls s \!+\! \Rs){F_1(s)}^{-1}\big{)}^{-1}{F_3(s)}.
\end{split}
\end{equation}
%from equations \eqref{eqn:omega_ml} and \eqref{eqn:T3}.
%\\The equation for $\frac{T_{\text{m}}}{\omega_{\text{m}}}$ given by \ref{eqn:6} and can be simplified further as shown below:
%\begin{equation}
%\label{eqn:10}
%\begin{aligned}
%\\\frac{T_{\text{m}}}{\omega_{\text{m}}}(s) =  %\frac{1}{T_1(s)} = \frac{D(s)}{J_{\text{l}} s^2 + %B_{\text{ml}} s + K_{\text{s}}} \\
%= \frac{(J_{\text{m}} s +B_{\text{m}}) (J_{\text{l}} s^2 + B_{\text{ml}} s + K_{\text{s}}) + J_{\text{l}} B_{\text{m}}s^2 + J_{\text{l}}K_{\text{s}}s}{J_{\text{l}} s^2 + B_{\text{ml}} s + K_{\text{s}}} \\
%= (J_{\text{m}} s +B_{\text{m}})+\bigg(\frac{J_{\text{l}} B_{\text{m}}s^2 + J_{\text{l}}K_{\text{s}} s}{J_{\text{l}} s^2 + B_{\text{ml}} s + K_{\text{s}}}\bigg)\\
%= (J_{\text{m}} s +B_{\text{m}})+ J_{\text{l}} s \times \underbrace{\Bigg(\frac{1}{1+\Big(\frac{J_{\text{l}} s^2 + (B_{\text{ml}}-B_{\text{m}}) s}{ B_{\text{m}}s + + K_{\text{s}}}\Big)}\Bigg)}_{\approx 1}\\
%&\approx ((J_{\text{m}}+J_{\text{l}}) s %+B_{\text{m}})
%\end{aligned}
%\end{equation}
Moreover, if $K_{\text{s}} \gg 1 $, one can approximate $F_1(s)^{-1}$ by $((J_{\text{m}}+J_{\text{l}}) s +B_{\text{m}})$.
%\begin{equation}
%T_1(s)^{-1} = 
%\frac{D(s)}{J_{\text{l}} s^2 + B_{\text{ml}} s + K_{\text{s}}}
%\approx ((J_{\text{m}}+J_{\text{l}}) s +B_{\text{m}}).
%\end{equation}
%\begin{equation}\begin{split}
%{F_1(s)^{-1}} 
%&= (J_{\text{m}}+J_{\text{l}}) s +B_{\text{m}} - \frac{J_{\text{l}}^2s^3}{J_{\text{l}} s^2 + B_{\text{ml}} s + K_{\text{s}}}\\&
%\approx ((J_{\text{m}}+J_{\text{l}}) s +B_{\text{m}}).
%\end{split}\end{equation}
This approximation is valid for the low range of frequencies, typically $[0,10^5]$ Hz, which includes the main frequency range of the operation of the system. 
The final transfer function is 
\begin{equation}\label{eqn:11}
\begin{split}
\!\!\!\!
G(s) &=  
\Kt \bigg{(}\Kt \Kb + \big{(}\Ls s+ \Rs\big{)}\big{(}(J_{\text{m}}+J_\mathrm{l}) s +B_{\text{m}}\big{)}\bigg{)}^{-1}
\!\!\!\!\!
\\
& \qquad \qquad 
\bigg({\frac{B_{m\mathrm{l}} s + K_{\text{s}}}{J_\mathrm{l} s^2 + B_{m\mathrm{l}} s + K_{\text{s}}}}\bigg).
\end{split}
\end{equation} 
%Figure \ref{fig:MotorandAxis} shows the transfer function block diagram representation of the motor and linear axis drive.
%\begin{figure}
%  \includestandalone[width=6.5cm]{Figures/MotorandAxi%s}
%  \caption{Transfer function block diagram of the motor and drive}
%  \label{fig:MotorandAxis}
%\end{figure}

\subsection{The Control Scheme}
\label{sec:control}
\begin{figure}[b]
\vspace{-4mm}
	\centering
	\includegraphics[width=0.485\textwidth]{Figs/ClosedLoop6.pdf}% 
	\caption{Block diagram of the system}
	\label{fig:Block2}
\end{figure}

The system is controlled by a PLC that runs a custom-made software package named LASAL.
The controller consists of three cascaded loops as shown in Figure  \ref{fig:Block2}, where 
%each loop regulates a different attribute of the system. In each control loop,
the output signals of each outer loop serves as the reference for the next inner loop. The first block in the axis controller is the interpolation block that receives the trajectory specifications from the user and determines the references for the position and the speed in the system. The interpolation block requires four inputs: position setpoint,  speed setpoint,  desired acceleration and desired deceleration. Once these inputs are provided, the interpolation block generates a reference speed and position trajectory using the equations of motion. The outer-most control loop is for linear position control. The middle control loop regulates the linear speed. 
The output of the interpolation block provides these loops with the designed nominal reference for the position and  the feed-forward reference for the speed. The motor encoder detects the position of the motor and  provides the feedback for both the position and speed control loops.
%The controller in the position control loop, denoted by $P(s)$, is a P-controller, whereas the controller in the speed control loop, denoted by $S(s)$, is a PI-controller %. More precisely, we have
%\begin{align}
%&P(s) = K_\text{p},\label{eqn:P(s)}\\
%&S(s) = K_\text{v} + \frac{K_\text{i}}{s}. \label{eqn:S(s)}
%\end{align}
The controller in the position control loop is a P-controller as $C_\text{p}(s) = K_\text{p}$, whereas the controller in the speed control loop, is a PI-controller as 
%$S(s) = K_\text{v} + \frac{K_\text{i}}{s}$.  
$C_\text{s}(s) = K_\text{v} + K_\text{i}/s$.  
One can also introduce $C_\text{v}(s)$ in the form of 
$C_\text{s}(s)=\Kv (1+1/\Tn(s))$ where $\Tn$ is the integral time constant of the controller.  The speed control loop provides the reference for the current controller, which is the inner-most loop.
The feedback in this loop is the measured current of the armature.
This loop is regulated by a PID-controller block %, denoted by $C(s)$, which is given as
denoted by
%begin{align}
%$C(s) = K_\text{{cp}} + \frac{K_\text{{ci}}}{s}  + K_\text{{cd}} s.$ 
$C_\text{c}(s) = K_\text{{cp}} + K_\text{{ci}}/s  + K_\text{{cd}} s.$ 
%\label{eqn:C(s)}
%\end{align}
The output of the controller is the voltage setpoint for the motor given to the motor drive. 
%The motor voltage is regulated according to this set reference via a motor drive system that converts the voltage reference to a corresponding input voltage for the motor. 
%As seen from the equation \ref{eqn:2}, current is directly related to the torque as a result of which the current controller is used to overcome torque disturbances and increase the effective electrical time constant. The speed controller moderates the acceleration and jerk (rate of change of acceleration) and consequently, the rate at which the system approaches the set position thereby attenuating the overshoot and hunting effect~\cite{stackex}. It also stabilizes the system in the presence of inertia and allows for a slower primary controller. Despite the effectiveness of the two inner loops, the primary position controller is essential and cannot be eliminated because it handles disturbances that may not affect the inner loops and provides the ability to change the position set point and adjusts the desired speed according to the position error \cite{cascaded2}.\par
%The last block in Figure \ref{fig:Block2} converts the rotational velocity of the ball-screw to linear speed. The factor $Q$ is the linear displacement of one complete rotation of the motor.
Finally, the last block in Figure \ref{fig:Block2} is not part of the controller but is used to convert the rotational velocity of the ball-screw to linear speed. The factor $Q$ is the linear displacement resulting from one complete rotation of the motor.

The linear axis has three separate modes of operation according to which control loops and parameters are chosen. In position control mode (used in this work), all three feedback loops are active and the position is the critical attribute of the system. In this mode, the controller will try to
adhere as close as possible to the position reference even if that entails deviating from the speed trajectory. In the speed control mode (not considered here), the speed trajectory is prioritized,
and the position controller deactivated by setting the gain in
the position controller to zero, $\Kp = 0$. 
Finally, in the current control mode (also not considered here), only the inner-most loop is active and the other controller gains are set to zero.
\begin{table}[t]
	\caption{Parameters of the current controller and the plant.}
	\label{table:motor_Parameters}
	\centering
	\ra{1.3}
	\begin{tabular}[h]{@{}l c c c c c  @{}}\toprule
		\multicolumn{2}{c}{Controller $C(s)$}  &&   \multicolumn{2}{c}{Plant}\\
		\cmidrule{1-2} \cmidrule{3-5}
		Parameter  &  Value && Parameter  &  Value  \\ \midrule
		$K_\text{{cp}}$ & $60$ && $\Rs$  & $9.02$ $\Omega$	\\ 
		$K_\text{{ci}}$ & $1000$ 	&& $\Ls$  & $0.0187$   \\
		$K_\text{{cd}}$ & $18$ && $K_{\text{t}}$  & $0.515$ Vs $\text{rad}^{{-1}}$ \\ 
		&&& $K_{\text{b}}$  & $0.55$ Nm $\text{A}^{-1}$\\ 
		&&& $J_{\text{m}}$  & $0.27\times 10^{-4} \text{ kg m}^2$  \\
		&&& $B_{\text{m}}$  & $0.0074$  	\\ 
		&&& $J_\text{l}$ &  $6.53 \times 10^{-4}\text{kg m}{}^2$ \\ 
		&&& $B_\text{{ml}}$ &  $0.014$ 			\\
		&&& $K_\text{s} $ &  $3 \times 10^7$ 	\\ 
		&&& $Q$ &  $1.8\times 10^{-2}$ m 	\\ 
		&&& Max. Speed   & $8000$ RPM  	\\
		\bottomrule 
	\end{tabular}
\end{table}
\subsection{The Parameters of the Model}
The transfer function of the plant as well as the control loops depend on several parameters. 
As our work concentrates on tuning the parameters of $C_\text{p}(s)$ and $C_\text{s}(s)$, it is assumed that the parameters of $C_\text{c}(s)$ are given. 
Values for most of the parameters of the plant are provided or can be calculated from the available data sheets. The only exception is $K_{\text{s}}$. We estimate this parameter experimentally by fitting  the step response of the model using least squares. The resulting parameter values are summarised in Table \ref{table:motor_Parameters}.

==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/sec_05_BO_tuning.tex <==
\section{Performance-Based Controller Tuning: Numerical Investigation}\label{sec:num_results}
\subsection{Classical Tuning Methods} \label{sec:classical_tuning_methods}
The numerical study provided in this section elucidates various aspects and features of the proposed data-driven controller tuning method and compares its performance to widely used tuning techniques. The classical PID tuning approach is the Ziegler-Nichols method, a heuristic designed for disturbance rejection \cite{ziegler1942optimum}, and an automated method where the controller is replaced by a relay and the PID coefficients are estimated based the resulting oscillatory response of the system \cite{hang2002relay}.
Other tuning approaches are also used in practice, where a performance indicator of the system response is minimized, e.g., the {\em integral of time-weighted absolute error} (ITAE) \cite{aastrom1993automatic}.

\subsection{Performance-Based Tuning Method}
\label{sec:performance_based_tuning_methods}
The performance-based tuning proposed here utilizes Bayesian optimization to tune the controller parameters (see Figure \ref{fig:scheme}). 
The main ingredient in Bayesian optimization is the cost function, which is composed of a set of metrics capturing the performance requirements of the system. For a linear actuator, in addition to the standard controller tuning metrics such as overshoot and settling time, the position tracking accuracy and the suppression of mechanical vibrations known as oscillation effects are of highest importance. 

%---------------------------------------------
\begin{figure}[h]
\vspace{-2mm}	\begin{subfigure}{.5\textwidth}
		\centering%.9
		\includegraphics[width=.65\linewidth]{Figs/metric_position_06.pdf}%  
%		\caption{Performance metrics in position tracking.}
		\label{fig:perf_metric_posi}
	\end{subfigure}
    \vspace{0mm}\\
	\begin{subfigure}{.5\textwidth}
		\centering%.86
		\includegraphics[width=.625\linewidth]{Figs/metric_speed_07.pdf}%
%		\caption{Performance metrics in speed tracking.}
		\label{fig:perf_metric_speed}
	\end{subfigure}
	\caption{The figure demonstrates various performance metrics for position tracking (top) and speed tracking (bottom). The reference  and the observed trajectory are shown respectively 
	by the red line and
	black line.}
	\label{fig:perf_metrics}
\end{figure}
%---------------------------------------------

Let the vector of controller gains be set to $\vc{x} := [\Kp,\Kv,\Ki]^\tr$ and an experiment be performed in time interval  $I:=[t^{\text{(i)}},t^{\text{(f)}}]$ with these gains. Once the experiment is completed,  the corresponding error signals for position,  $\ep: I\to\Rbb$, and for speed, $\es: I\to\Rbb$, are measured, and used to calculate the tracking performance metric for $\vc{x}$. %denoted by $f(\vc{x})$ below. 

%The tracking performance $f$ is consisted of two parts, one for tracking the position reference, denoted by $\fp$, and  one for tracking the speed reference, denoted by $\fs$. Both $\fp$ and $\fs$ are weighted sums of different quantities where each of them reflects a feature of tracking the reference trajectories and the weights depend on the scale and the importance of corresponding features. For the performance in position tracking,

For position tracking, the corresponding performance metrics are the overshoot, $\hp$, the undershoot, $\hpu$, the steady-state error, $\epSS$, the settling time, $\Tp$, and the maximum absolute position error (infinity norm), $\| \ep\|_{\infty}$. To minimize oscillations due to the excitation of vibration modes, the integral of the time-weighted absolute value of the error of the position response also defined \cite{aastrom1993automatic} as
%\begin{equation}
$\ep_{\text{ITAE}} := \int_{{t^{\text{(i)}}}}^{t^{\text{(f)}}} (t-t^{\text{(i)}})|\ep(t)|\ \mathrm{d}t$,
%\end{equation}
is  also included. 
The {\em position zero error}, $\epZERO$,  is defined as the error of the system once it returns to zero position (zero) once the motion is completed and it is of high interest, as it quantifies the oscillations in the system.
The same metrics are also used for the speed tracking error
and superscript `(s)' is used to denote the corresponding speed metrics.
%For the performance in speed tracking, we consider similar metrics such as the overshoot, $\hs$, the undershoot, $\hsu$, the steady-state error, $\esSS$, the settling time of the speed step response, $\Ts$, the infinity norm of tracking error, $\| \es \|_{\infty}$, and the time-weighted absolute value of the error of the speed response, $\es_{\text{ITAE}}$, for considering the oscillations due to the excitation of vibrational modes. %As discussed in Section \ref{sec:problem_statement}, 
%Beside these performance metrics, we may consider other additional ones. In fact, the choice of a particular performance metrics is based on its impact on the close-loop response of the system. For example, minimizing the steady state error $\esSS$ results in achieving the desired speed set point. Also, $\hsu$ is a measure of the jerk and should be minimized to prevent damaging the structure.
%-----------------------------------------------
\iffalse 
\begin{table}[t]
	\caption{Weights for the cost function of the position and the speed  controllers}
	\centering
	\ra{1.3}
	\begin{tabular}[h]{ @{}l c c c c c c c @{} }\toprule
		\multicolumn{2}{c}{position}  &&&   \multicolumn{2}{c}{speed}\\
		\cmidrule{1-4} \cmidrule{5-7}
		$\Fp_i$   & $\gammap$ &&&  $\Fs_i$ & $\gammas$ \\ \midrule %\hline
		$\Tp$ & $10^4$              &&& $\Ts$ & $500$ &\\ %\hline
		$\hp$ & $10$                &&& $\hs$ & $2$ & \\ %\hline  
		$\hpu$ & $0$                &&& $\hsu$ & $0$ & \\ %\hline  
		$\ep_{\text{ITAE}}$& $0$    &&& $\es_{\text{ITAE}}$ & $10^4$ & \\ %\hline 
		$\|\ep\|_{\infty}$ & $100$  &&& $\|\es\|_{\infty}$ & $500$ &\\
		$\epSS$ & $0$               &&& $\esSS$ & $0$ & \\ %\hline  
		$\epZERO$ & $0$             &&& && \\ %\hline 
		\midrule 
		$\alphap$ & $10$             &&& $\alphas$&$1$& \\ %\hline 
		\bottomrule
	\end{tabular}	
	\label{table:weights_grid}
\end{table}   
\else 
\begin{table}[b]
\centering
\vspace{-4mm}
	\ra{1.3}
	\begin{tabular}[h]{ @{}l c c c c c c c @{} }\toprule
		\multicolumn{2}{c}{position}  &&&   \multicolumn{2}{c}{speed}\\
		\cmidrule{1-4} \cmidrule{5-7}
		$\Fp_i$   & $\gammap$ &&&  $\Fs_i$ & $\gammas$ \\ \midrule %\hline
		$\Tp$ & $10^5$              &&& $\Ts$ & $5\cdot 10^2$ &\\ %\hline
		$\hp$ & $10^2$                &&& $\hs$ & $2$ & \\ %\hline  
		$\|\ep\|_{\infty}$ & $10^3$  &&& $\|\es\|_{\infty}$ & $5\cdot 10^2$ &\\
		& &&& $\es_{\text{ITAE}}$ & $10^4$ & \\ %\hline 
%		\midrule 
%		$\alphap$ & $1$             &&& $\alphas$&$1$& \\ %\hline 
		\bottomrule
	\end{tabular}	
	\caption{Weights in the cost function 
	%of the position and the speed controllers
	}\label{table:weights_grid}
\end{table}   
\fi
%--------------------------------------------------

We take a weighted sum of the individual position metrics, denoted by $\Fp_i(\vc{x}), i=1,\ldots,\Np$, with corresponding weights $\gammap_i, i=1,\ldots,\Np$,  to generate a combined position metric $\fp(\vc{x})$. Similarly, we generate a combined speed metric, denoted by $\fs(\vc{x})$. In order to generate an overall performance metric for controller tuning, 
we then take sum of the two quantities as
$f(\vc{x}):=\fp(\vc{x})+\fs(\vc{x})$. 
%we then take a weighted sum of the two quantities as \begin{equation}\label{eqn:perf} f(\vc{x}):=\alphap\fp(\vc{x})+\alphas\fs(\vc{x}),    \end{equation} where $\alphap$ and $\alphas$ are the trade-off factors. 
The values of the different weights used are summarised in Table \ref{table:weights_grid}.
\iffalse%-------------------------------------------
Define vectors $\Fp=[\Fp_i]_{i=1}^{\Np}$ and $\Fs=[\Fp_i]_{i=1}^{\Ns}$ as
\begin{equation}
\Fp := [\hp,\hpu,\Tp,\| \ep\|_{\infty},\ep_{\text{ITAE}},\epSS,\epZERO]^\tr, \label{eqn:Fp}
\end{equation}
and
\begin{equation}
\Fs := [\hs,\hsu,\Ts,\| \es\|_{\infty},\es_{\text{ITAE}},\esSS]^\tr, \label{eqn:Fs}
\end{equation}
where $\Fp_i$ and $\Fs_i$ are respectively the $i^{\text{\tiny{th}}}$ entry of $\Fp$ and the $i^{\text{\tiny{th}}}$ entry of $\Fs$, and $\Np$ and $\Ns$ are respectively the length of $\Fp$ and the length of $\Fs$. Here, we have $\Np=7$ and $\Ns=6$.
Let $\gammap :=[\gammap_i]_{i=1}^{\Np}$ and $\gammas :=[\gammas_i]_{i=1}^{\Ns}$ be respectively the weights for different performance metrics in position and speed tracking.
Therefore, $\fp$ and $\fs$ are defined as
\begin{equation}\label{eqn:fp_and_fs_linear_sum}
\fp = \sum_{i=1}^{\Np}\gammap_i\Fp_i, \qquad
\fs = \sum_{i=1}^{\Ns}\gammas_i\Fs_i.
\end{equation}
Accordingly, the overall performance metric or cost objective is defined as 
\begin{equation}\label{eqn:perf}
f(\vc{x}):=\alphap\fp(\vc{x})+\alphas\fs(\vc{x}),    
\end{equation}
where $\alphap$ and $\alphas$ are the trade-off factors.
The weight vectors $\gammap$ and $\gammas$ as well as the trade-off factors $\alphap$ and $\alphas$ are given in Table \ref{table:weights_grid}. 
\fi%-------------------------------------------
Each  of the weights depends on the scale and the importance of corresponding metric and feature and can be selected considering the particular application requirements, e.g. maximization of tracking accuracy in position, minimization of response time, or  minimization of oscillations in the system. 


A fundamental constraint for tuning the controllers is the stability of the closed-loop system during the tuning procedure. This can be achieved by constraining the controller gains to known ranges guaranteeing this feature. 
To this end, the feasible set for $\vc{x}$, denoted by $\Xcal$, is defined as
%\begin{equation}\label{eqn:X_gains_range}
%\!\!\!
%\Xcal\!:=\! 
%[K_{\text{p},\min},\!K_{\text{p},\max}] 
%\!\!\times\!\!
%[K_{\text{v},\min},\!K_{\text{v},\max}] 
%\!\!\times\!\!
%[K_{\text{i},\min},\!K_{\text{i},\max}], \!\!\!
%\end{equation}
\begin{equation}\label{eqn:X_gains_range}
\begin{split}
%\Xcal&:=\\ 
&[K_{\text{p},\min},\!K_{\text{p},\max}] 
\!\times\!
[K_{\text{v},\min},\!K_{\text{v},\max}] 
\!\times\!
[K_{\text{i},\min},\!K_{\text{i},\max}], \!
\end{split}
\end{equation}
where $K_{\text{p},\min}$,  
$K_{\text{v},\min}$ and  
$K_{\text{i},\min}$ are the smallest positive values acceptable by the controller,  
$K_{\text{p},\max} = 4200$,  
$K_{\text{v},\max} = 0.5$,  and
$K_{\text{i},\max} = 900$.
In practice, these ranges are either provided with the system, or estimated in a safe exploration procedure. Here, we have derived them by a grid computation of the system response for various controller parameters.

%----------------------------
\begin{algorithm}[t]
	\caption{Performance-based Tuning Method}\label{alg:performace_based_tuning}
	\begin{algorithmic}[1]
		\State \textbf{Input:} Set $\Xcal$ (see \eqref{eqn:X_gains_range}), training data set, $\Dcal_0$, and trade-off weights $\gammap$, $\gammas$.
		\State Estimate the vector of hyperparameters $\hat{\theta}$.
		\State $\Dcal\leftarrow \Dcal_0$ and $m\leftarrow m_0$.
		\While{stopping condition is not met}
		\State Update the GP model: calculate $\mu_m$ and $\sigma_m$. % using \eqref{eqn:mu} and \eqref{eqn:sigma}.
		\State Derive $\vc{x}_{m+1}$ by solving \eqref{eqn:GP_LCB}.
		\State Update $\Kp$, $\Kv$ and $\Ki$, run experiment and measure signals $\ep_{m+1}$ and $\es_{m+1}$.
		%\State Calculate the performance metrics $\Fp$ and $\Fs$ (see \eqref{eqn:Fp} and  \eqref{eqn:Fs})
		\State Calculate the measured performance $y_{m+1}$.
		\State $\Dcal\leftarrow \Dcal \cup \{(\vc{x}_{m+1},y_{m+1})\}$ and $m\leftarrow m+1$.
		\EndWhile\label{DCP_loop}
		\State \textbf{end} 
		\State \textbf{Output:} $\vc{x}_{\mBO^*}$.
	\end{algorithmic}
\end{algorithm}%\vspace{-3mm}
%----------------------------
Note that $\fp$, $\fs$ and $f$ are functions of controller gains $\vc{x}$ in an {\em oracle form}.  The controller parameters with optimal performance, $\vc{x}^*$, are the ones inducing  minimum cost objective $f$. 
To find these optimal values, we utilize Bayesian optimization, summarized in Algorithm \ref{alg:performace_based_tuning}. 
Starting from feasible set $\Xcal$, we perform a sequence of experiments. 
In the $m^{\text{\tiny{th}}}$ experiment, a new vector of controller gains $\vc{x}_m$ is used, and based on the measured error signals, the corresponding performance 
$ f(\vc{x}_m)$ is evaluated as $y_m$.
The first $m_0$ experiments are for constructing the initial data set 
$\Dcal_0:=\{(\vc{x}_m,y_m)|m=1,2,\ldots,m_0\}$.  
%While it is possible to start the Algorithm from an initial empty set of data, an initial informative data set improves the tuning procedure.
Using GPR and the collected data, we obtain a surrogate function for the performance metric $f$ as a Gaussian process $\GP{\mu_m}{k_m}$, where $\mu_m:\Xcal\to\Rbb$ is the mean function predicting the value of $f$ at different locations, and $k_m:\Xcal\!\times\!\Xcal\to\Rbb$ is the kernel function evaluating the uncertainty in the predictions.
Here, we utilize {\em squared exponential} kernel with hyperparameters tuned  using $\Dcal_0$.
The controller gains are updated due to GP-LCB sampling algorithm \cite{srinivas2012information} as
\begin{equation}\label{eqn:GP_LCB}
\vc{x}_{m+1}=\argmin_{\vc{x} \in \Xcal}\ \mu_{m}(\vc{x})-\beta_{m}\sigma_{m}(\vc{x}) \, 
\end{equation}
where 
$\sigma_{m}(\vc{x}):=k_{m}(\vc{x},\vc{x})$ indicates the variance in prediction of performance function at $\vc{x}$ and 
$\beta_{m}$ is a constant specifying the considered confidence bound around the mean function $\mu_m$.
%%<---
\iffalse
Finally, one should note that a fundamental constraint for tuning the controllers is the stability of the closed-loop system during the tuning procedure. This can be achieved by constraining the controller gains to known ranges guaranteeing this feature.  To this end, the feasible set for $\vc{x}$ is defined as
\begin{equation}\label{eqn:X_gains_range}
\!\!\!
\Xcal\!:=\! 
[K_{\text{p},\min},\!K_{\text{p},\max}] 
\!\!\times\!\!
[K_{\text{v},\min},\!K_{\text{v},\max}] 
\!\!\times\!\!
[K_{\text{i},\min},\!K_{\text{i},\max}], \!\!\!
\end{equation}
where $K_{\text{p},\min}$,  
$K_{\text{v},\min}$ and  
$K_{\text{i},\min}$ are the smallest non-negative positive values acceptable by the controller,  
$K_{\text{p},\max} = 4200$,  
$K_{\text{v},\max} = 0.5$,  and
$K_{\text{i},\max} = 900$.
In practice, these ranges are either provided by the company that manufactured the system or they can be estimated by performing a safe exploration procedure. Here, we have derived the ranges based on a numerical procedure in which the response of system is computed for various choices of the controller parameters, and subsequently the stability is ensured. 
\fi
This procedure stops at iteration $\mBO$ either by reaching the maximum number of iterations, or by sampling around the same configuration of parameters with minimal cost more than three times.
The output of the algorithm is the vector of controller gains with the best observed performance, $\vc{x}_{\mBO^*}$.


One could also tune the gains of the two loops sequentially, alternating between the gains of the inner and the outer loop, utilizing BO for each step \cite{IFACBOCascade}. We do not pursue this direction further here, since the combined tuning approach introduced above is more likely to lead to a globally optimal solution.
%\begin{remark}
%Similar to the classical methods for tuning cascade control structures, one may utilize a performance-based sequential tuning approach \cite{IFACBOCascade}.
%In other words, first the controller gains in outer loop is set to a nominal value and the controller in the inner loop is tuned. Following this, the gains in the inner loop is set to the tuned values and the controller in the outer loop is tuned. This back-and-forth procedure is continued until the controller gains converge.
%More precisely, we split the vector of controller gains $\vc{x}$ into $\xp:=[\Kp]$, for position control loop, and $\xs := [\Kv,\Ki]^\tr$, for speed control loop. First, $\xp$ is set to the nominal value $\xp_1$ and $\xs$ is tuned such that the speed tracking performance objective is optimized, i.e., we optimize $\fs(\xp_1,\xs)$ with respect to $\xs$ by performing a sequence of experiments and utilizing Bayesian optimization. Let the final obtained gain vector be denoted by $\xs_1$. Following this, $\xs$ is set to $\xs_1$ and $\xp$ is tuned such that the position tracking performance metric is optimized, i.e., we optimize $\fp(\xp,\xs_1)$ with respect to $\xp$ in a similar manner. Let the obtained value be denoted by $\xs_2$. This procedure is repeated until reaching to a stopping condition like maximum allowed number of iterations. Note that in this sequential tuning procedure, we need to employ a sequence of Bayesian optimization procedures. Moreover, there is no theoretical guarantee for the convergence of tuning procedure. Accordingly, we only focus here on the former presented method.	
%\end{remark}



%\begin{figure}[b]
%	\centering
%	\includegraphics[width=0.45\textwidth]{Figs/3dres1a.png}
%	\caption{The figure shows the values of performance cost function on the grid. The training samples (black points) and the result of performance-based tuning (red point) are shown. One can see that the performance-based result is in the region of optimal performance.}
%	\label{fig:costs}
%\end{figure}


\subsection{Numerical Experiments} \label{sec: BO_sim}
%In the numerical experiments, we take the feasible set of the controller gains, $\Xcal$, as given in \eqref{eqn:X_gains_range} and use the transfer function model as outlined in Section \ref{sec:system_model} to generate system trajectories (as shown in Figure \ref{fig:perf_metrics}) and hence evaluate the cost for different gain values in $\Xcal$. 
We now compare the system trajectories of the transfer function model from Section \ref{sec:system_model} corresponding to BO tuning, classical methods, and an exhaustive (grid) computation of the performance metric on a $280 \times 90 \times 100$ grid on $\Xcal$. %In the process, we observed that in the vicinity of the the optimal gains, the performance is almost identical to the optimum performance, suggesting that the graph of the performance function is roughly flat in the region around the optimal gains with optimum performance. 
To apply Algorithm \ref{alg:performace_based_tuning}  we initialize with dataset $\Dcal_0$ collected from random locations in $\Xcal$. In each iteration, we solve the GP-LCB optimization problem \eqref{eqn:GP_LCB} by calculating the objective function of \eqref{eqn:GP_LCB} for the points of the grid and finding the point with the optimal cost; note that this process does not require data to be collected at all the grid points, only that the Gaussian process is evaluated at these points.
Table \ref{table:SimCompare} shows that the controller gains, as well as the performance resulting from the proposed method are almost the same as the performance of optimal grid point, i.e., the performance-tuning method finds the controller gains in the nearly flat region of performance around the optimal gains.
\begin{table}[t]
\vspace{-1mm}		
\caption{Results of different tuning methods}
	\label{table:SimCompare}
	\centering
	\ra{1.3}
	\begin{tabular}[h]{@{}l c c c c c  @{}}\toprule
		Tuning method  &  $\Kp$ &  $\Kv$ &  $\Ki$ & $f$\\ \midrule
		Grid search (true optimal value)&225&0.39&90& 4557\\ 
		Ziegler Nichols &392&0.18&510 & 28434\\  
		ITAE criterion&255&0.11&420 & 31163 \\ 
		Relay Tuning&115&0.05&130& 23396 \\ 
		%		Sequential Bayesian optimization &225&0.37&130\\
		Performance-based Tuning &240&0.39&100& 4586\\ \bottomrule
	\end{tabular}
\vspace{-4mm}	
\end{table}

\begin{figure}[t]
	\centering
	\includegraphics[width=0.485\textwidth]{Figs/allTracesJoint2.pdf}
	\caption{Response for different benchmark tuning methods}
	\label{fig:benchmark}
	\vspace{-6mm}
\end{figure}

The closed-loop speed and position responses corresponding to benchmark tuning methods to the performance-based tuning responses, namely Zeigler-Nichols method, relay tuning, and ITAE in Figure \ref{fig:benchmark} show significantly higher overshoot and oscillations compared to the performance-based tuning responses, which also matches the ideal response obtained by grid simulation. The position response tracks the input reference precisely, and the speed response has a slight overshoot in the acceptable range.
Table \ref{table:SimCompare} shows the resulting control gains and corresponding performance. The result of the performance-based tuning is closest to the exhaustive evaluation results obtained on the grid while the gains obtained via standard tuning approaches (Zeigler-Nichols, relay tuning, and ITAE) are more aggressive.
The number of training samples in $\Dcal_0$ has a direct influence on the number of iterations needed to reach the stopping criterion that defines the converged controller gains. A more informed prior model requires less iterations during the optimization phase.
We further performed a Monte Carlo simulation, where the algorithm was initialized with a different number of data points selected randomly from $\Xcal$, and for each value of $m_0$ Algorithm 1 was executed 1000 times for a maximum number of 60 iterations.
Based on these numerical experiments, 
%shown in Table \ref{table:monte_carlo}, 
an initial data set $\Dcal_0$ comprising 20-50 different random configurations of parameters requires a tuning phase of $20$ up to $50$ iterations in total for convergence, which is a reasonable trade-off between the number of initial samples and tuning phase iterations.
Since the performance metrics can be fully automated, and the initial exploration phase needs to be repeated only upon major changes in the system, the proposed tuning method can be efficiently implemented.
The numerical experiments are useful to clarify several open points in the performance-based autotuning, even though tuning on the real system does not require a model and is purely data-driven. First, the numerical experiments give an initial, safe indication if the method is working or not. Second, they indicate how many training points we should expect in realty to have a reasonable number of iterations for convergence. Similarly, they indicate the number of iterations need for convergence, and finding a suitable stopping criterion. Finally, they provide the range of stability in the controller gains. If the stability range is unknown, and if unstable parameters cannot be detected in advance, the application in reality might bring failures in the system. The method applied in practice is not influenced by the model or by the optimal parameters found in numerical experiments, as it provides the true optima according to the corresponding convergence criteria.
 

==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/sec_10_exper.tex <==
\section{Performance-Based Controller Tuning: Experimental Results} \label{sec:experimental}
%This section demonstrates the performance-based BO controller tuning 
%on a linear motion stage. It's performance and robustness are evaluated for different loads, presence of disturbances, and for various reference trajectories.
%\subsection{Experimental Set-up and Settings}
The linear motion system (stage) used to validate the proposed tuning method consists of a linear axis, a permanent magnet AC motor with a servo drive, and a Programmable Logic Controller (PLC), as shown in Figure \ref{mfig:structure}. The system is equipped with a linear encoder with a precision of $1\mu\text{m/m}$ and sampling time of $1\text{ms}$ used for measuring the actual position and speed of the stage. The input voltage to the motor is provided based on the voltage reference signal from a Sigmatek S-DIAS PLC. 
Since the bandwidth of the current controller is above $1500\text{Hz}$ and the corresponding bandwidth of the position controller does not exceed $400\text{Hz}$, the current closed-loop can be well approximated with a constant gain. The proportional controller gains $\Kv$ and $\Kp$ of the cascade control loop are tuned, and the integral time constant $\Tn$ is tuned instead of the the integral gain $\Ki$.

For the joint tuning of the control parameters, the input setpoints (position, speed, acceleration, deceleration) were set identical for each run of the system. During the experiments, acceleration and deceleration values were kept high to simulate step input and step response in both position and speed control modes, and the speed was set at $20\frac{\text{cm}}{\text{s}}$. The range of the three control parameters was limited following the numerical experiments to ensure that the system is always  in a stable mode: $K_\text{p} \in (0,65000], K_\text{v} \in (0,7000], T_\text{n} \in (1000,40000]$.
%--------------------------------------------------
\iffalse 
\begin{table}[t]
	\caption{Weights for the cost function of the position and the speed  controllers}
	\centering
	\ra{1.3}
	\begin{tabular}[h]{ @{}l c c c c c c c @{} }\toprule
		\multicolumn{2}{c}{position}  &&&   \multicolumn{2}{c}{speed}\\
		\cmidrule{1-4} \cmidrule{5-7}
		$\Fp_i$   & $\gammap$ &&&  $\Fs_i$ & $\gammas$ \\ \midrule %\hline
		$\Tp$ & $20$                 &&& $\Ts$ & $20$ &\\ %\hline
		$\hp$ & $50000$              &&& $\hs$ & $1000$ & \\ %\hline  
		$\hpu$ & $0$                &&& $\hsu$ & $2000$ & \\ %\hline  
		$\ep_{\text{ITAE}}$& $0$    &&& $\es_{\text{ITAE}}$ & $250000$ & \\ %\hline 
		$\|\ep\|_{\infty}$ & $50000$ &&& $\|\es\|_{\infty}$ & $0$ &\\
		$\epSS$ & $0$               &&& $\esSS$ & $500$ & \\ %\hline  
		$\epZERO$ & $10^5$          &&& && \\ %\hline 
		\midrule 
		$\alphap$ & $1$            &&& $\alphas$&$1$& \\ %\hline 
		\bottomrule
	\end{tabular}	
	\label{table:weights_grid_exp}
\end{table}
\else
\begin{table}[b]
\vspace{-4mm}	
	\centering
	\ra{1.3}
	\begin{tabular}[h]{ @{}l c c c c c c c @{} }\toprule
		\multicolumn{2}{c}{position}  &&&   \multicolumn{2}{c}{speed}\\
		\cmidrule{1-4} \cmidrule{5-7}
		$\Fp_i$   & $\gammap$ &&&  $\Fs_i$ & $\gammas$ \\ \midrule %\hline
		$\Tp$ & $2\cdot 10^1$                 &&& $\Ts$ & $2\cdot 10^1$ &\\ %\hline
		$\hp$ & $5\cdot 10^4$              &&& $\hs$ & $10^3$ & \\ %\hline  
		%\hline 
		$\|\ep\|_{\infty}$ & $5\cdot 10^4$ &&& $\es_{\text{ITAE}}$ & $2.5\cdot 10^5$ &\\
		$\epZERO$ & $10^5$               &&& $\esSS$ & $5\cdot 10^2$ & \\ %\hline  
		&                &&& $\hsu$ & $2\cdot 10^3$ & \\ %\hline  
%	    \midrule 
%		$\alphap$ & $1$            &&& $\alphas$&$1$& \\ %\hline 
		\bottomrule
	\end{tabular}	
		\caption{Weights in the cost function% of the position and the speed  controllers
	}
	\label{table:weights_grid_exp}
\end{table}
\fi 
%--------------------------------------------------

The position reference trajectory was a bi-directional step response, where the nut moves from  $0$ to $50$cm, remains there for $10$s, and returns to position $0$. In this case, input position and speed are set to $5$cm and $100\frac{\text{cm}}{s}$, respectively. 
The modified weights used in the experimental implementation of the performance-based tuning are provided in Table \ref{table:weights_grid_exp}. The termination criterion for tuning in practice was based on either achieving a predefined number of iterations, or reaching a minimum within a defined threshold and sampling at this candidate configuration for at least $3$ iterations. 



 



%\begin{figure}[b]
%	\centering
%	\includegraphics[width=0.49\textwidth]{Figs/figureBO1.pdf}
%	\caption{GP model of the objective function (performance $f$) after convergence,  the corresponding training samples (black dots) and final sampling point (white circle).}
%	\label{fig:ExperBO_cost_samples}
%\end{figure}

  

%\begin{table}[t]
%	\caption{Results of Monte Carlo Simulations with 1000 runs}
%	\centering
%	\ra{1.3}
%	\begin{tabular}[h]{ @{}l c c c c c c c @{} }\toprule
%		& \multicolumn{2}{c}{Perf.- based Tuning}  &&   \multicolumn{2}{c}{Perf.-based Tuning with noise}\\
%		\cmidrule{1-4} \cmidrule{5-7}
%		& Mean  & Std. Dev && Mean  & Std. Dev \\ \midrule %\hline
%		$\Kp$ & 253.75 & 21.44               && 259.55 & 25.36 &\\ %\hline
%		$\Kv$ & 0.386 & 0.0265              && 0.386 & 0.0263 & \\ %\hline  
%		$\Ki$ & 94 & 11.6                && 94.6 & 11.65 & \\ %\hline  
%		$\mTRAIN$ & 34.5 & 9   &&   &  & \\ %\hline 
%		$\mBO $ & 28.5 & 11.5    &&  &  & \\ %\hline 
%		$\mBO + \mTRAIN$ & 63 & 11.9    && 64.5 & 12.5 & \\ %\hline 
%		Cost $f$ & 4641.3 & 78.1  && 4638 & 94.45 &\\
%		\bottomrule
%	\end{tabular}	
%	\label{table:monte_carlo}
%\end{table}  




\subsection{Experimental Results: Performance and Robustness}

\begin{figure}[h]
	\centering
	\includegraphics[width=0.425\textwidth]{Figs/BO_system_exper.pdf}
	\caption{Position and speed responses comparing tracking traces of the system optimized with performance-based BO tuning and traces corresponding to the nominal parameters optimized by manual tuning. The insets show the initial overshoot obtained with each method.}
	\label{fig:ExperBO_grid}
	\vspace{-4mm}
\end{figure}



Initially, $49$ samples were obtained for different values of $\Kp$, $\Kv$ and $\Tn$. 
The required performance metrics were extracted from each of the data sets and the corresponding cost was calculated for each configuration of gains. 
Tuning the parameters using these training data for computing priors results in convergence after $18$ iterations. %The resulting predicted posterior mean of the cost is shown on Figure \ref{fig:ExperBO_cost_samples}.
The optimal point is reached after repeated sampling near the optimum of the cost. The optimal values for the position and speed controller obtained are $\Kp = 44500$, $\Kv = 4000$ and $\Tn = 12500$. The system response in position control mode using the above controller configuration for set position of $50$cm and set speed of $50 \frac{\text{cm}}{\text{s}}$ is shown in Figure \ref{fig:ExperBO_grid}.
The negligible oscillation on the response is due to the amplified noisy resolver feedback, observed also in the nominal configuration. The speed response in the position control mode shown in Figure \ref{fig:ExperBO_grid} also has an overshoot of $14$\% which is higher than the speed control mode as expected but is within an acceptable range with a maximum speed of $57.5\frac{cm}{s}$. This is also in part due to the noise of the system. The position response steady state error is significantly smaller as compared to that in nominal mode, and the overshoot in position is less than $0.2$cm with very fast settling so there is no tracking delay or error.
 Performance-based tuning achieves better tracking and lower overshoot for both speed and position modes, and faster settling time for the more important position control mode. The results are summarized in Table \ref{table:expResults}, where it can be seen that the optimized parameters have reached higher values than the parameters from nominal tuning for the same load.

\begin{table}[b]
\vspace{-4mm}
	\centering
	\ra{1.1}
	\begin{tabular}[h]{@{} c c c c c c c  @{}}\toprule
		&$ $& $\Kp$ & $\Tn$ & $\Kv$  &$\fp$&$\fs$\\ 
		&$\mBO$ & $\!\times10^2$ & $\!\times10^2$ & $\!\times10^2$ & $\!\times10^3$  & $\!\times10^3$ \\ \midrule
		Nominal (no load) & - & 200 & 100 & 25 & 523 & 271\\
		Perf.-based (no load) & 67 & 445 & 125 & 40 & 401.9 & 224.9 \\
		Perf.-based (extra load) & 43 & 650 & 130 & 42.5 & 254.2 & 281.8 \\
		\bottomrule 
	\end{tabular}
\caption{Summary of all tuning results on the linear drive 
	}	
\label{table:expResults}
\end{table}


Because of the large number of samples in the training phase, the cost evolution during the BO iterations starts from a very low estimated cost, but with high uncertainty, and moves to higher cost, where the uncertainty is reduced after $10$ iterations, as shown in Figure \ref{fig:BOexpCost_evolution}. Looking at the {\em current minimal} cost, it can be seen that the BO-based tuning reaches a low-uncertainty cost which is very close to the converged results already at iteration 5. The algorithm converges after 18 iterations, according to the specified somewhat conservative termination criterion.
\begin{figure}[h]
	\centering
    \includegraphics[width=0.35\textwidth]{Figs/Exp_cost_evolutionNoPriors.pdf}
      \caption{Predicted,   actual   observed   cost,   and   associated confidence interval at  3  standard  deviations  for  performance-based  BO  tuning on the system.}	\vspace{-5mm}
  \label{fig:BOexpCost_evolution}
\end{figure}

We have further tested the robustness of the tuning approach by providing reference trajectories with different profiles. Figure \ref{fig:BOExpTraj} shows that the performance achieved with the BO tuning exceeds the nominal performance when there are fast changes in the speed, as in the top panels, and achieves better tracking of the references. The speed undershoot is significantly reduced, and better position stability is achieved at standstill, which is an important performance requirement for linear motion systems. For the trajectories shown in the bottom panels of Figure \ref{fig:BOExpTraj} the performance is virtually the same as nominal. 

\begin{figure}[b]
\vspace{-4mm}
	\centering
    \includegraphics[width=0.475\textwidth]{Figs/Nominal_trajectories_Optimized.pdf}
      \caption{Position and speed responses comparing tracking with different trajectories. Upper panels: Position and speed responses for different step signals; Bottom panels: Trajectories with varying speed setpoints. 
      %In all cases, the performance of the proposed method is better.
      }
  \label{fig:BOExpTraj}
\end{figure}

Standard tuning methods such as the Ziegler-Nichols rule or relay tuning show excellent performance for disturbance rejection objectives. We have evaluated the BO-based controller parameters with respect to disturbance rejection. Impulsive disturbance forces were applied during the operation in the direction of movement of the system with additional load. The resulting response is shown in Figure \ref{fig:expDisturb}, and compared with the system's nominal performance when subjected to the same type of disturbance. The response of the system shows a quick recovery following the disturbance, as shown in Figure \ref{fig:expDisturb}. Even though the applied disturbance has significantly higher magnitude than in the nominal case, the observed recovery is faster for the performance-based tuned controller gains. This is due to the performance metric term that corresponds to tracking accuracy and position stability.

\begin{figure}[b]
	\centering
	\vspace{-4mm}
	\includegraphics[width=0.45\textwidth]{Figs/DisturbanceCombined.pdf}
	\caption{Speed responses of the system without and additional load, comparing disturbance response of the nominal controller and the BO-optimized controller.}
	\label{fig:expDisturb}
\end{figure} 
 
\iffalse 
\subsection{Performance-Based Tuning With Additional Load}

When there is a change in the load, the controller gains can be re-tuned. Here, we add a cylinder attached to the table breadboard on the linear axis with $9$ kg weight and re-tune the controller gains using the same performance objective function. The new tuning results in better performance, as shown in Figure \ref{fig:BOexpLoad}. The tuned controller results are provided in Table \ref{table:expResults}. The main difference here is the higher proportional gain $\Kp$ of the position controller. Adjusting for the modification in the system results in both reducing the overshoot in the speed response, and reducing the settling time for the position tracking. For the re-tuning, $10$ samples were used in training, and convergence was achieved in $33$ iterations. We have further investigated the effect of re-tuning with a different prior, i.e., the one from the system without an additional load. Then the optimization continues until the maximal set number of iterations is reached. However, when the minimum cost of the prior is taken into account, the optimization can be stopped %at any time 
when good performance with respect to the prior is achieved.   
\begin{figure}[t]
	\centering
    \includegraphics[width=0.475\textwidth]{Figs/compare_withLoad.pdf}
      \caption{Position and speed responses comparing tracking of the system, for performance-based tuned controller parameters with and without with an additional load. The insets show the overshoot obtained with each method.}
  \label{fig:BOexpLoad}
\end{figure}
\fi 
 
\subsection{Discussion} 
The proposed performance-based BO tuning thus offers a trade-off between grid based search, and heuristic-based methods. With BO tuning a relatively small number of experiments leads to the optimal gains, specified according to the data-driven optimization objective and termination criterion. The number of experiments can be varied, and usually prior experiments can be significantly reduced while achieving good performance.
Currently, tuning is performed in specified ranges to avoid destabilizing values of the parameters. The ranges are derived either based on the model of the system or based on expert knowledge from operating the system. When the ranges are not a priori known, and for the full automation of the method, it would be useful to ensure a safety mechanism in the performance-based tuning procedure. This could be achieved either through the addition of the safety constraints such as Gaussian processes in the BO algorithm or through the modification of the acquisition function to account for the probability of constraint violation \cite{Maier2019}. Another possibility is to detect experimentally when the system is approaching critical regime and to include a safety penalty in the cost \cite{SafetyBO2020}.
%Exhaustive evaluation requires extensive number of experiments to evaluate all parameter combinations, and provides the optimal gains (according to a fixed criterion), whereas standard tuning methods, including model-based tuning (e.g. symmetric optimum) require significantly reduced number of experiments, but often result in conservative gains. 

==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/sec_97_conclusion.tex <==
\section{Conclusion and Outlook} \label{sec:conclusion}
%In this paper, we have presented a data-driven approach for cascade controller tuning in which the performance of a closed-loop system is modeled as function of controller gains. Due to the oracle form of the performance function, a Bayesian optimization approach is utilized to derive controller gains with optimal performances. 
%For verifying the efficiency of the method, we have taken a ball-screw linear axial system. First, by modeling the plant and deriving the parameters of the model, the tuning method was evaluated numerically and compared to classical tuning approaches, as well as to exhaustive evaluation. The method was then implemented on the real plant and its efficiency was investigated experimentally.
%Based on the observed results, the method enables fast and standardized tuning, with a performance superior to other auto-tuning approaches and is guaranteed to converge. Furthermore, it enables easy adaptation of the controller parameters upon changes in the load, or in the mechanical configuration of the system. Also, the proposed method enables tuning the controller while the system is in normal operation mode. Extending the method with automatic detection of instabilities, or safe exploration in the evaluation of the cost will further extend its flexibility and potential for practical use.
We have presented a data-driven approach for cascade controller tuning, where we model the performance of a closed-loop system as a function of controller gains. We apply a Bayesian optimization approach to derive controller gains with optimal performance. The performance was first evaluated in a simulation for a ball-screw linear axial system,  and compared to classical tuning approaches and the computed optimal performance on a grid. 
The experimental validation of the proposed method shows that it enables fast and standardized tuning, with a performance superior to other autotuning approaches. 
It allows easy adaptation of the controller parameters upon changes in the load or the system's mechanical configuration. Extending the method with automatic detection of instabilities will further increase its flexibility and potential for practical use.
%\vspace{-1cm}

%due to the oracle form of the performance function

%Extending the method with automatic detection of instabilities, or safe exploration in the evaluation of the cost

==> Performance-Driven Cascade Controller Tuning with Bayesian Optimization - short version 2/sec_98_ackno1.tex <==
\section{Acknowledgement}
The authors gratefully acknowledge Sigmatec AG for providing technical assistance with the LASAL software, as well as the linear axis drive system and the associated PLC.

==> sec_03_preli.tex <==
\section{Gaussian Processes and Bayesian Optimization} \label{sec:GP_BO}
%Bayesian optimization is a data-driven approach for solving optimization problems where the objective function is unknown and available in form of a noisy {\em oracle}. 
%BO samples and learns the objective function efficiently online by querying the oracle for different candidate configurations of inputs. BO uses Gaussian process regression (GPR) iteratively to build a surrogate for the objective function and quantify the associated uncertainty~\cite{BayesOpt4} for all possible configurations. In each iteration, the data is used for deciding on the next evaluation point based on an acquisition function. 
%The new information, the result of queried oracle on the new evaluation point, is combined with the prior knowledge using Gaussian process regression to estimate the objective function, and to find its minimum~\cite{BayesOpt4}, corresponding to the optimal input configuration. 
\subsection{Gaussian Processes}
\label{GP}
A Gaussian process (GP) is a collection of random variables where each of its finite subsets is jointly Gaussian \cite{GPR}. 
The GP is uniquely characterized by the mean function, $\mu:\Xcal \to \Rbb$, and the  covariance/kernel function, $k:\Xcal\times\Xcal\to \Rbb$, where $\Xcal$ is the set of location indices.
The GP is denoted by $\GP{\mu}{k}$ %or $\GP{\mu(\cdot)}{k(\cdot,\cdot)}$
, $\Xcal$ is a subset of $\Rbb^d$ and the kernel is the {\em square exponential} kernel
\begin{equation}
k_{\text{SE}}(\vc{x},\vc{x}') \!=\!
\sigma_{f}^2\exp{\bigg{(}\!\!-\!\frac{1}{2}(\vc{x}\!-\! \vc{x}')^{\tr}\mathrm{L}^{-1}(\vc{x}\!-\!\vc{x}')\!\bigg{)}},
\end{equation}
for any $\vc{x},\vc{x}'$ in $\Xcal$ where $\sigma_f$ and $\mathrm{L}$ 
% and $\sigma_n$ 
are the hyperparameters of the kernel, respectively referred as {\em length scale matrix} and {\em flatness parameter}. % and {\em noise variance}, and $\delta_{\vc{x},\vc{x}'}$ is {\em Kronecker delta} function, i.e.,  $\delta_{\vc{x},\vc{x}'}=1$, if $\vc{x}=\vc{x}'$ and $\delta_{\vc{x},\vc{x}'} = 0$, otherwise. 

Gaussian processes provide flexible models for Bayesian learning by introducing prior distributions  over the space of functions defined on $\Xcal$.
Due to the favorable properties of the Gaussian distributions, the marginal and the conditional mean and variance can be computed on any finite set of locations in a closed form. 
%Subsequently, a probabilistic  non-parametric regression  method can be developed \cite{GPR}.
%More precisely, let $f:\Xcal\to\Rbb$ be an unknown function, $\GP{\mu}{k}$ be the prior distribution for estimating $f$, and noisy measurements at locations $\vcc{x} := \begin{bmatrix}\vc{x}_1& \vc{x}_2 &\ldots &\vc{x}_m\end{bmatrix}$ be given as  $\vcc{y} := \begin{bmatrix}\vc{y}_1& \vc{y}_2 &\dots& \vc{y}_m\end{bmatrix}^\tr\in\Rbb^m$. 
Let $f:\Xcal\to\Rbb$ be an unknown function, $\GP{0}{k}$ be the prior distribution for estimating $f$, and noisy measurements at locations $\vc{x}_1,\ldots,\vc{x}_m$ be respectively given as  $\vc{y}_1,\dots,\vc{y}_m$. 
In other words, we know that $f\sim \GP{0}{k}$ and  $\vc{y}_i=f(\vc{x}_i)+w_i$, for $i=1,\ldots,m$, where $w_i$ is the measurement noise with zero mean Gaussian distribution $\Ncal(0,\sigma_w^2)$. 
Since there is no additional information about the latent function $f$, we can set the mean of the GP prior to zero. 
Let $\vc{x}\in\Xcal$ be a new location where the corresponding measurement is not provided. 
Since the joint distribution of the measurements data is Gaussian with a given mean and a given covariance, one can predict the value of measurement at the new location $\vc{x}$ using {\em Bayes rule}. 
First, we define $\mx{X}_m$ and $\vc{y}_m$ respectively as $\mx{X}_m:= [\vc{x}_1,\vc{x}_2,\ldots,\vc{x}_m]\in\Rbb^{n\times m}$ and $\vc{y}_m := [y_1,y_2,\ldots,y_m]^\tr\in\Rbb^m$.
Also, we define the Gram matrix $\mathrm{K}_{{\mx{X}_m\mx{X}_m}}\in\Rbb^{m\times m}$ such that its  element at the $i^{\text{\tiny{th}}}$ row and the $j^{\text{\tiny{th}}}$ column is given by $k(\vc{x}_i,\vc{x}_j)$. 
Consequently, due to $f\sim \GP{0}{k}$, we know that 
$\vc{y}_m \sim \Ncal\big{(}\zero,\mx{K}_{\mx{X}_m\mx{X}_m}+\sigma^2_w\eye\big{)}$, where $\eye$ denotes the identity matrix.
%\begin{equation}
%     \mathrm{y} \sim \mathcal{N}\bigg{(}0,\mathrm{K}_{\mathrm{xx}}+\sigma^2_n\mathbb{I}\bigg{)} \,.
%\end{equation}  
The joint distribution of the training data $\{(\vc{x}_i,y_i)\}_{i=1}^m$ with the new data point $(\vc{x},y_\vc{x})$, where  $y_\vc{x} := f(\vc{x})$ is the unknown label for location $\vc{x}$, can be calculated as 
\begin{equation}
    \begin{bmatrix}
    \vc{y}_m\\y_\vc{x}
    \end{bmatrix} \sim \mathcal{N}\bigg{(}0,\begin{bmatrix} \mx{K}_{\mx{X}_m\mx{X}_m} + \sigma^2_w\eye & \vc{k}_{\vc{x}\mx{X}_m}^\tr \\ \vc{k}_{\vc{x}\mx{X}_m} & k_{\vc{x}\vc{x}} \end{bmatrix}\bigg{)}  \,,
\end{equation} 
where $\mathrm{k}_{\vc{x}\mx{X}_m}\in\Rbb^m$ is the vector such that its $i^{\text{\tiny{th}}}$ element is given by the kernel as $k(\vc{x},\vc{x}_i)$, for any $i=1,\ldots,m$, and $ k_{\vc{x}\vc{x}}:=k(\vc{x},\vc{x})$. The posterior distribution of $y_{\vc{x}}|\mx{X}_m,\vc{y}_m$ is a Gaussian distribution as
\begin{equation}
    y_{\vc{x}} | \mx{X}_m,\vc{y}_m \sim \mathcal{N}(\mu_m(\vc{x}),\sigma_m(\vc{x})) \,,
\end{equation}
where the mean of prediction, $\mu_m(\vc{x})$, and the corresponding covariance, $\sigma_m(\vc{x})$, are given as 
\begin{align}
\mu_m(\vc{x}) &:= \vc{k}_{\vc{x}\mx{X}_m}^\tr\big{(}\mx{K}_{\mx{X}_m\mx{X}_m}+\sigma^2_w\eye\big{)}^{-1}\vc{y}_m,
\label{eqn:mu}\\
\sigma_m(\vc{x}) &:= k_{\vc{x}\vc{x}} - \mathrm{k}_{\vc{x}\mx{X}_m}^\tr\big{(}\mathrm{K}_{\mx{X}_m\mx{X}_m}+\sigma^2_w\eye\big{)}^{-1}\vc{k}_{\vc{x}\mx{X}_m}. \label{eqn:sigma}
\end{align}
The posterior mean $\mu_m(\vc{x})$ is a nonlinear function predicting the value of $f$ at location $\vc{x}$ with an uncertainty  described by $\sigma_m(\vc{x})$. Accordingly, this is a nonlinear non-parametric regression method called {\em Gaussian process regression} (GPR).
%The GPR depends on hyperparameters such as .
The hyperparameters of the kernel $\sigma_f$, $\mx{L}$ and $\sigma_w$ collected in a vector $\theta\in\Theta$ can be estimated by minimizing the negative log marginal log-likelihood of the joint distribution of the training data,
\begin{equation}\label{eqn:min_nlml}
\hat{\theta}:= 
\argminOp_{\theta\in\Theta}\ -\log p(\mathrm{y}_m|\mx{X}_m,\theta) \, ,
\end{equation}
where $ p(\mathrm{y}_m|\mx{X}_m,\theta)$ is the probability density function of the labels or measurements acquired at locations $\{\vc{x}_i\}_{i=1}^m$. 
%________________________________
%________________________________
\subsection{Bayesian Optimization Algorithm}
The goal of Bayesian optimization is to find efficiently a solution for the problem
\begin{equation}\label{eqn:x_star_argmin_f}
\vc{x}^* = \argminOp_{\vc{x}\in\Xcal}\ f(\vc{x}) \,,
\end{equation} 
where $f:\Xcal\to \Rbb^n$ is an unknown function that is expensive to evaluate, available only as a noisy {\em oracle}. In the optimization \eqref{eqn:x_star_argmin_f},  $\vc{x}$ can be a vector of design parameters or decision variables. Similarly, $f$ can be a user-defined cost function or a specific designed performance indicator.

In Bayesian optimization, the information about the unknown objective is collected by efficient on-line sampling and querying the oracle, and subsequently, learning the unknown function and deriving the global optimal solution iteratively. %More precisely, a set of sampling points is generated sequentially for which the oracle is queried.
For any $m\in\Nbb$, let $\vc{x}_m\in\Xcal$ and $y_m\in\Rbb$ denote respectively the $m^{\text{\tiny{th}}}$ sampling point and the corresponding value returned by the oracle.
 Since the oracle is noisy, we have $y_m = f(x_m)+w_m$, where $w_m$ is the evaluation noise of oracle.
 In each sampling iteration $m\in \Nbb$, a surrogate function is learned for the unknown objective function using Gaussian process regression and the associated uncertainty is quantified, using \eqref{eqn:mu} and \eqref{eqn:sigma}.
 %At iteration $m\in \Nbb$, given noisy measurements  $y_1,\dots,y_m$ respectively for sampling locations $\vc{x}_1,\ldots,\vc{x}_m$,
%using Gaussian process regression, one can obtain the posterior distribution and also,  $\mu_m$ and $\sigma_m$ as in \eqref{eqn:mu} and \eqref{eqn:sigma}.
Accordingly, $\mu_m$ is the surrogate function and $\sigma_m$ quantifies the corresponding uncertainty in the prediction of the value of objective function on the future sampling point.
The next candidate evaluation point $\vc{x}_{m+1}$
is determined based on a sampling criterion called {\em acquisition function}. 
Commonly used acquisition functions include \textit{entropy search}, \textit{expected improvement}, \textit{upper confidence bound (UCB)}, etc~\cite{BayesOpt4}.
The acquisition function provides a trade-off between exploitation and exploration.  %It can explore regions of the domain with maximum information and highest prediction uncertainty, exploit the point with the lowest predicted cost or select new locations according to a combination of these two objectives~\cite{srinivas2012information}. 
Here we use the {\em lower confidence bound} (LCB) of the predicted objective function~\cite{srinivas2012information}, defined as 
\begin{equation}\label{eqn:GP_LCB}
\vc{x}_{m+1}=\argminOp_{\vc{x} \in \Xcal}\ \mu_{m}(\vc{x})-\beta_{m}\sigma_{m}(\vc{x}) \, ,
\end{equation}
where
$\beta_{m}$ is a constant specifying the considered confidence bound around the mean function $\mu_m$. The LCB acquisition function selects points $\boldsymbol{x}$ with large uncertainty $\sigma_{m}$ and with low cost prediction $\mu_{m}$. %It implicitly negotiates the exploration - exploitation trade-off.
A natural interpretation of this sampling rule is that it greedily selects points $\vc{x}$ where $f(\vc{x})$ could be lower than the current minimum and upper bounds the function by the current minimum \cite{srinivas2012information}.

Let $m^*$ be the index of sampling point with minimum observed cost amongst $\vc{x}_1,\ldots,\vc{x}_m$, i.e., 
\begin{equation}\label{eqn:mstar}
m^* = \argmin_{i\in\{1,2,\ldots,m\}}y_i.    
\end{equation}
While it is guaranteed that as $m$ goes to infinity, the uncertainty is reduced and the best observed point, $\vc{x}_{m^*}$, converges to the $\vc{x}^*$, we need to introduce a finite-time practical stopping criterion ~\cite{srinivas2012information}. 
%The suitable criteria are case-dependent and need to be decided based on the underlying application and the system specifications. 
Since the primary goal is to reduce the number of evaluations, the stopping condition used here is limiting the number of iterations to be less than a predefined maximum number, denoted by $\mBO$. %An additional stopping criterion is introduced to reduce further the number of iterations.
When sampling occurs repeatedly around the current minimum, the algorithm is terminated after three successive iterations. The stopping criteria are flexible and can be determined according to the specific applications of the tuning algorithm.

==> sec_98_ackno1.tex <==
\section{Acknowledgement}
The authors gratefully acknowledge Sigmatec AG for providing technical assistance with the LASAL software, as well as the linear axis drive system and the associated PLC.
